CUDA-L1: Improving CUDA Optimization via Contrastive Reinforcement Learning

The exponential growth in demand for GPU computing resources has created an urgent need for automated CUDA optimization strategies. While recent advances in LLMs show promise for code generation, current SOTA models achieve low success rates in improving CUDA speed. In this paper, we introduce CUDA-L1, an automated reinforcement learning framework for CUDA optimization that employs a novel contrastive RL algorithm. CUDA-L1 achieves significant performance improvements on the CUDA optimization task: trained on A100, it delivers an average speedup of x3.12 with a median speedup of x1.42 against default baselines over across all 250 CUDA kernels of KernelBench, with peak speedups reaching x120. In addition to the default baseline provided by KernelBench, CUDA-L1 demonstrates x2.77 over Torch Compile, x2.88 over Torch Compile with reduce overhead, x2.81 over CUDA Graph implementations, and x7.72 over cuDNN libraries. Furthermore, the model also demonstrates portability across different GPU architectures. Beyond these benchmark results, CUDA-L1 demonstrates several properties: it 1) discovers a variety of CUDA optimization techniques and learns to combine them strategically to achieve optimal performance; 2) uncovers fundamental principles of CUDA optimization, such as the multiplicative nature of optimizations; 3) identifies non-obvious performance bottlenecks and rejects seemingly beneficial optimizations that actually harm performance. The capabilities demonstrate that, RL can transform an initially poor-performing LLM into an effective CUDA optimizer through speedup-based reward signals alone, without human expertise or domain knowledge. This paradigm opens possibilities for automated optimization of CUDA operations, and holds promise to substantially promote GPU efficiency and alleviate the rising pressure on GPU computing resources.

==> header_style.tex <==
% 一次性加载 geometry，给出页边距和 \headheight
% 增加 headsep 来让第一页页眉和正文之间有更大间距
\usepackage[margin=3cm, headheight=50pt, headsep=0pt]{geometry}

\usepackage{graphicx}   % 插图
\usepackage{fancyhdr}   % 自定义页眉页脚

% ------- 页眉定义 -------
\pagestyle{fancy}       % 默认页眉样式
\fancyhf{}              % 清空

% 删除默认页面的横线
\renewcommand{\headrulewidth}{0pt}

\begin{comment}
% 左侧：logo + 项目名，可按需删掉 \textsc{}
\fancyhead[L]{%
  \raisebox{-0.25\height}{\includegraphics[height=20pt]{./header.png}}%
}

% 右侧放页码示例（可不要）
\fancyhead[R]{}

% (2) 横向"拉长"：把页眉区域往左右各伸出 2.5 cm
\fancyheadoffset[L]{0.2cm}
\fancyheadoffset[R]{0.2cm}
\end{comment}

% 让首页 (plain) 同样使用这种页眉
\fancypagestyle{plain}{%
  \fancyhf{}
  \fancyhead[L]{%
    % 方法1：通过添加 \vspace 来让页眉内容下移
    \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{\includegraphics[height=25pt]{./header.png}}%
      \vfill
    }%
  }
  \fancyhead[R]{
  \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{}
      \vfill
    }%
  }
  \renewcommand{\headrulewidth}{0.7pt}  % 保留第一页的横线
  \fancyheadoffset[L]{0cm}
  \fancyheadoffset[R]{0cm}
}

% 如果只想让第一页的页眉和正文间距更大，可以在文档开始处使用：
% \thispagestyle{plain}
% \vspace{20pt}  % 在第一页正文开始前添加额外空间

==> images/avg_speedup_and_code_comparsion.tex <==


\begingroup                      
  \captionsetup[sub]{labelformat=figsub,labelsep=space,labelfont=footnotesize}
  \renewcommand\thesubfigure{\thefigure(\alph{subfigure})}
  
\begin{figure}[H]
    \centering
    % 左侧柱状图区域
    \begin{minipage}[t][6cm][c]{0.33\textwidth}  % 减小左侧宽度
    %
        \centering
       %\vspace{0.1cm}
       \adjustbox{max width=\textwidth, max height=6cm,center}{
            \includegraphics[scale=7]{./images/general_result_all_level_v2.png}
        }
       % \vspace{0.1cm}
        \subcaption[]{\scriptsize Average speedup across different architectures on KernelBench.}
        %\vspace{0.1cm}
    \end{minipage}
    %\hfill
    % 右侧代码区域
    \begin{minipage}[t][6cm][c]{0.58\textwidth}  % 增加右侧宽度
        \centering
        % 优化前的代码
       \begin{adjustbox}{scale=0.92}
        \begin{tcolorbox}[
            rounded corners,
            enhanced,
            width=1\textwidth,
            colframe=codegreen,
            colback=white,
            title=\textbf{ diag(A) * B | Reference Code},
            fonttitle=\bfseries\footnotesize,
            left=0pt,   % 适当的左边距
            right=0pt,  % 适当的右边距
            top=0pt,
            bottom=0pt,
        ]
        \begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none, framerule=0pt, escapeinside={(*@}{@*)}, keywordstyle=\color{templateblue}\bfseries, showspaces=false, showstringspaces=false, breaklines=true, breakatwhitespace=true]
class Model(nn.Module):   
   def forward(self, A, B):
       # A: (N,) - 1D tensor of shape N
       # B: (N, M) - 2D tensor of shape N x M
       # torch.diag(A): (N, N) - creates diagonal matrix from A
       # Result: (N, N) @ (N, M) = (N, M)
       return torch.diag(A) @ B
        \end{lstlisting}
        \end{tcolorbox}
        \end{adjustbox}
        \vspace{-0.3cm}
        % 优化后的代码
        \begin{adjustbox}{scale=0.92}
        \begin{tcolorbox}[
            rounded corners,
            arc=2pt,
            enhanced,
            width=1\textwidth,
            colframe=codegreen,
            colback=white,
            title=\textbf{ diag(A) * B | CUDA-L1 Implementation (64x faster)},
            fonttitle=\bfseries\footnotesize,
            left=0pt,   % 适当的左边距
            right=0pt,  % 适当的右边距
            top=0pt,
            bottom=0pt,
        ]
        \begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none, framerule=0pt, escapeinside={(*@}{@*)}, keywordstyle=\color{templateblue}\bfseries, showspaces=false, showstringspaces=false, breaklines=true, breakatwhitespace=true]
class Model(nn.Module):   
   def forward(self, A, B):
       return A.unsqueeze(1) * B
        \end{lstlisting}
        \end{tcolorbox}

        \end{adjustbox}
        \vspace{0.2cm}
        \subcaption[]{\scriptsize A case from KernelBench (Level 1, Task 12), computing \texttt{diag(A) * B}. We present reference code and CUDA-L1 implementation. The CUDA-L1 implementation reduces complexity from $O(N^2M)$ to $O(NM)$, achieving {\bf 64\times} speedup by replacing full matrix multiplication with element-wise operations.}
        \end{minipage}
    \label{fig:optimization}
\end{figure}
\endgroup  

==> images/exp_different_gpus_levels.tex <==
\begin{table*}
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.1}
\begin{tabular}{@{}lc|cccc|cc@{}}
\toprule[1.2pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{8}{c}{\textbf{Level 1}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{GPU Device}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & \small{\# out of 100} & \small{\# out of 100} \\
\midrule
A100 PCIe & \textbf{2.78} & 65.8 & \textbf{1.75} & \textbf{1.28} & \textbf{1.12} & \textbf{99} & \textbf{94} \\
H100 & 1.83 & 20.0 & 1.43 & 1.14 & 1.02 & \textbf{99} & 83 \\
L40 & 2.52 & \textbf{108} & 1.50 & 1.16 & 1.02 & \textbf{99} & 89 \\
RTX 3090 & 2.21 & 65.0 & 1.38 & 1.11 & 1.01 & 98 & 80 \\
H20 & 2.08 & 35.3 & 1.38 & 1.16 & 1.02 & \textbf{99} & 87 \\
\midrule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{8}{c}{\textbf{Level 2}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{GPU Device}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & \small{\# out of 100} & \small{\# out of 100} \\
\midrule
A100 PCIe & 3.55 & 120 & \textbf{2.05} & 1.39 & 1.20 & \textbf{100} & \textbf{98} \\
H100 & 2.79 & 81.9 & 1.67 & 1.38 & 1.16 & 99 & 96 \\
L40 & \textbf{4.02} & \textbf{182} & 1.76 & 1.37 & 1.16 & 99 & 93 \\
RTX 3090 & 3.10 & 114 & 1.57 & 1.27 & 1.07 & 94 & 87 \\
H20 & 2.69 & 63.7 & 1.69 & \textbf{1.42} & \textbf{1.20} & 99 & 97 \\
\midrule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{8}{c}{\textbf{Level 3}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{GPU Device}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & \small{\# out of 50} & \small{\# out of 50} \\
\midrule
A100 PCIe & \textbf{2.96} & 24.9 & 2.60 & \textbf{1.94} & \textbf{1.42} & \textbf{50} & 48 \\
H100 & 2.78 & 15.9 & 3.13 & 1.81 & 1.32 & 49 & 48 \\
L40 & 2.58 & \textbf{32.3} & 2.31 & 1.74 & 1.25 & \textbf{50} & 46 \\
RTX 3090 & 2.19 & 18.4 & 2.44 & 1.53 & 1.13 & \textbf{50} & 46 \\
H20 & 2.40 & 8.45 & \textbf{3.36} & 1.84 & 1.40 & 49 & \textbf{49} \\
\bottomrule[1.2pt]
\end{tabular}
\caption{CUDA-L1 performance on KernelBench across different GPU devices for levels 1, 2 and 3.}
\label{gpu-level-results}
\end{table*}

==> images/general_result.tex <==
\begin{figure*}[!h]
\vspace{-0.15cm}
 \centering
 \begin{adjustbox}{margin=-0.5cm 0cm 0cm 0cm}
 \begin{minipage}[c]{\textwidth}
 \centering
\includegraphics[scale=0.35]{./images/general_result.png}
\caption{Average speedup achieved by CUDA-L1 across different architectures on KernelBench.}
\label{fig:general_result}
 \end{minipage}
 \end{adjustbox}
 \end{figure*}

==> images/general_result_plot.tex <==
\begin{figure*}[!h]
\vspace{-0.15cm}
 \centering
 \begin{adjustbox}{margin=-0.5cm 0cm 0cm 0cm}
 \begin{minipage}[c]{\textwidth}
 \centering
\includegraphics[scale=0.4]{./images/general_result_plot_img.png}
\caption{Average speedup comparisons on KernelBench across different level subsets}
\label{fig:general_result_plot}
 \end{minipage}
 \end{adjustbox}
 \end{figure*}

==> images/plot_all_levels.tex <==
%\vspace{-1cm}
\begin{figure*}
 \centering
 \begin{adjustbox}{margin=-0.5cm 0cm 0cm 0cm}
 \begin{minipage}[c]{\textwidth}
 \centering
\includegraphics[scale=0.4]{./images/speedup_ratio.png}
\caption{Number of examples v.s. speedup ratio for different levels.}
\label{fig:plot_levels}
 \end{minipage}
 \end{adjustbox}
 \end{figure*}

==> tables/ablation_optim_case.tex <==
%\begin{table}[htbp]
%  \centering
  %============================= Outer container (single prompt)
  %\begin{adjustbox}{margin=-0.2cm 0cm 0cm 0cm, scale=0.9}
\newcommand{\bluecode}[1]{\textcolor{code-highlight-blue}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\greencode}[1]{\textcolor{code-highlight-green}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\yellowcode}[1]{\textcolor{code-highlight-yellow}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\purplecode}[1]{\textcolor{code-highlight-purple}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\redcode}[1]{\textcolor{code-highlight-red}{\bfseries\footnotesize\ttfamily #1}}

\captionof{table}{Reference code and CUDA-L1 generation for Bidirectional GRU class}
  
  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Bidirectional GRU | Reference Code - Simple baseline implementation},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries,]
class ModelReference(nn.Module):
    def __init__(self, input_size, hidden_size, num_layers=3, bias=True, batch_first=False):
        """
        Simple reference implementation - no optimizations
        """
        super(ModelReference, self).__init__()
        
        self.gru = nn.GRU(input_size, hidden_size, num_layers, }bias, batch_first, dropout=0, bidirectional=True)
        self.h0 = torch.randn((num_layers * 2, 10, hidden_size))  # batch_size=10
    
    def forward(self, x):
        """
        Basic forward pass with no optimizations
        """
        self.h0 = self.h0.to(x.device)
        output, h_n = self.gru(x, self.h0)
        return output

\end{lstlisting}
\label{tab:ablation-reference-code}
  \end{tcolorbox}


  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Bidirectional GRU | Fully Optimized Code - All optimizations enabled (400x faster)},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries, stringstyle = \color{black},]
import torch
import torch.nn as nn

# (*@\emoji{control-knobs}@*) ========== OPTIMIZATION TOGGLE SWITCHES ==========
# Change these True/False values to enable/disable optimizations
USE_CUDA_GRAPHS = True         # (*@\emoji{blue-circle}@*) CUDA graph capture and replay
USE_MEMORY_OPTIMIZATION = True # (*@\emoji{green-circle}@*) Pre-allocation and caching  
USE_STREAM_MANAGEMENT = True   # (*@\emoji{purple-circle}@*) Dedicated CUDA streams
USE_REDUCED_BRANCHING = True   # (*@\emoji{red-circle}@*) Minimal conditional logic

# (*@\emoji{cross-mark}@*) KERNEL WARMUP is EXCLUDED from this model
# =====================================================

class ModelNew(nn.Module):
    def __init__(self, input_size, hidden_size, num_layers=3, bias=True, batch_first=False):
        """
        Model with 4 optimizations (excluding kernel warmup)
        
        Edit the USE_* variables above to enable/disable optimizations
        """
        super(ModelNew, self).__init__()
        
        self.gru = nn.GRU(input_size, hidden_size, num_layers, bias, batch_first, 
                          dropout=0, bidirectional=True)
        
        # (*@\emoji{control-knobs}@*) OPTIMIZATION SWITCHES (from global variables)
        self.use_cuda_graphs = USE_CUDA_GRAPHS
        self.use_memory_optimization = USE_MEMORY_OPTIMIZATION
        self.use_stream_management = USE_STREAM_MANAGEMENT
        self.use_reduced_branching = USE_REDUCED_BRANCHING
        
        # Always have the base hidden state
        self.h0 = torch.randn((num_layers * 2, 10, hidden_size))  # batch_size=10
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS variables (always initialized for consistency)
        self.graph = None
        self.static_input = None
        self.static_h0 = None
        self.static_output = None
        self.static_hn = None
        self.expected_shape = None
        self.expected_device = None
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION variables
        self.graph_cache = {} if self.use_memory_optimization else None
        
        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT variables
        self.stream = None
        
        # (*@\emoji{red-circle}@*) REDUCED BRANCHING variables
        self.call_count = 0
        
        # Print configuration
        self._print_config()
    
    def _print_config(self):
        """Print current optimization configuration"""
        print("(*@\emoji{control-knobs}@*)  OPTIMIZATION CONFIGURATION:")
        print("(*@\emoji{blue-circle}@*) CUDA Graphs: " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_cuda_graphs else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{green-circle}@*) Memory Optimization: " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_memory_optimization else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{yellow-circle}@*) Kernel Warmup:   (*@\emoji{cross-mark}@*) OFF (EXCLUDED)")
        print("(*@\emoji{purple-circle}@*) Stream Management:  " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_stream_management else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{red-circle}@*) Reduced Branching:  " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_reduced_branching else "(*@\emoji{cross-mark}@*) OFF"))
        print("=" * 50)
    
    def _get_graph_key(self, x):
        """(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Generate unique key for graph caching (if enabled)"""
        if self.use_memory_optimization:
            (*@\greencode{return (x.shape, str(x.device))}@*)
        return None
    
    def _initialize_cuda_graph(self, x):
        """(*@\emoji{blue-circle}@*) CUDA GRAPHS: Initialize graph with conditional optimizations (no warmup)"""
        
        if not self.use_reduced_branching:
            print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Initializing CUDA graph...")
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Check cache first (if enabled)
        if self.use_memory_optimization:
            (*@\greencode{shape\_key = self.\_get\_graph\_key(x)}@*)
            (*@\greencode{if shape\_key and shape\_key in self.graph\_cache:}@*)
                (*@\greencode{cached\_data = self.graph\_cache[shape\_key]}@*)
                (*@\greencode{self.graph = cached\_data['graph']}@*)
                (*@\greencode{self.static\_input = cached\_data['input']}@*)
                (*@\greencode{self.static\_output = cached\_data['output']}@*)
                (*@\greencode{self.static\_h0 = cached\_data['h0']}@*)
                (*@\greencode{self.static\_hn = cached\_data['hn']}@*)
                (*@\greencode{self.expected\_shape = x.shape}@*)
                (*@\greencode{self.expected\_device = x.device}@*)
                if not self.use_reduced_branching:
                    print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Using cached graph")
                return
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Store expected characteristics
        self.expected_shape = x.shape
        self.expected_device = x.device
        
        # Create static tensors
        self.static_input = torch.zeros_like(x, device=x.device)
        
        if self.use_memory_optimization:
            #(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Use pre-allocated h0
            (*@\greencode{self.static\_h0 = self.h0.to(x.device).contiguous()}@*)
        else:
            # Create new h0 each time (less efficient)
            h0 = self.h0.to(x.device).clone()
            self.static_h0 = h0.contiguous()
        
        # Determine output shape
        if self.gru.batch_first:
            batch_size, seq_len = x.shape[:2]
            output_shape = (batch_size, seq_len, self.gru.hidden_size * 2)
        else:
            seq_len, batch_size = x.shape[:2]
            output_shape = (seq_len, batch_size, self.gru.hidden_size * 2)
        
        self.static_output = torch.zeros(output_shape, device=x.device)
        self.static_hn = torch.zeros((self.gru.num_layers * 2, batch_size, self.gru.hidden_size), 
                                    device=x.device)
        
        # (*@\emoji{cross-mark}@*) NO KERNEL WARMUP: Skip warmup - kernels will compile during graph capture
        # This may cause slower first execution
        
        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Create dedicated stream (if enabled)
        if self.use_stream_management and self.stream is None:
            (*@\purplecode{self.stream = torch.cuda.Stream()}@*)
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Capture the computation graph
        self.static_input.copy_(x)

        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Use dedicated stream
        if self.use_stream_management:
            (*@\purplecode{self.stream.wait\_stream(torch.cuda.current\_stream())}@*)
            (*@\purplecode{with torch.cuda.stream(self.stream):}@*)
                (*@\purplecode{self.graph = torch.cuda.CUDAGraph()}@*)
                (*@\purplecode{with torch.cuda.graph(self.graph):}@*)
                    # Use FP32 only - no mixed precision
                    (*@\purplecode{output, hn = self.gru(self.static\_input, self.static\_h0)}@*)
                    (*@\purplecode{self.static\_output.copy\_(output)}@*)
                    (*@\purplecode{self.static\_hn.copy\_(hn)}@*)
        else:
            # Use default stream
            self.graph = torch.cuda.CUDAGraph()
            with torch.cuda.graph(self.graph):
                # Use FP32 only - no mixed precision
                output, hn = self.gru(self.static_input, self.static_h0)
                self.static_output.copy_(output)
                self.static_hn.copy_(hn)
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Cache the graph (if enabled)
        if self.use_memory_optimization and shape_key:
            (*@\greencode{self.graph\_cache[shape\_key] = \{}@*)
                (*@\greencode{'graph': self.graph,}@*)
                (*@\greencode{'input': self.static\_input,}@*)
                (*@\greencode{'output': self.static\_output,}@*)
                (*@\greencode{'h0': self.static\_h0,}@*)
                (*@\greencode{'hn': self.static\_hn}@*)
            (*@\greencode{\}}@*)
            if not self.use_reduced_branching:
                print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Cached graph for shape " + str(x.shape))
    
    def forward(self, x):
        """
        Forward pass with configurable optimizations (no kernel warmup)
        """
        
        # (*@\emoji{red-circle}@*) REDUCED BRANCHING: Conditional debugging
        if not self.use_reduced_branching:
            (*@\redcode{self.call\_count += 1}@*)
            print("\n--- Forward pass #" + str(self.call_count) + " ---")
            print("Input shape: " + str(x.shape) + ", device: " + str(x.device))
        
        # Fast path for CPU
        if not x.is_cuda:
            h0 = self.h0.to(x.device)
            # Use FP32 only - no mixed precision
            output, _ = self.gru(x, h0)
            return output
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Contiguous check (if enabled)
        if self.use_memory_optimization and not x.is_contiguous():
            (*@\greencode{x = x.contiguous()}@*)
            if not self.use_reduced_branching:
                print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Made input contiguous")
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Try to use CUDA graphs (if enabled)
        if self.use_cuda_graphs:
            try:
                # Check if graph needs initialization
                (*@\bluecode{need\_init = (self.graph is None or }@*)
                           (*@\bluecode{self.expected\_shape != x.shape or}@*) 
                           (*@\bluecode{self.expected\_device != x.device)}@*) 
                
                (*@\bluecode{if need\_init:}@*)
                    (*@\bluecode{if not self.use\_reduced\_branching:}@*)
                        (*@\bluecode{print("\emoji{blue-circle} CUDA GRAPHS: Initializing graph")}@*)
                    (*@\bluecode{with torch.no\_grad():}@*)
                        (*@\bluecode{self.\_initialize\_cuda\_graph(x)}@*)
                
                # Execute with CUDA graph
                (*@\bluecode{self.static\_input.copy\_(x)}@*)
                
                if self.use_stream_management:
                    # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Execute in dedicated stream
                    (*@\purplecode{with torch.cuda.stream(self.stream):}@*)
                        (*@\purplecode{self.graph.replay()}@*)
                else:
                    # Execute on default stream
                    self.graph.replay()
                
                if not self.use_reduced_branching:
                    print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Graph executed successfully")
                
                return self.static_output
                
            except Exception as e:
                if not self.use_reduced_branching:
                    print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Failed (" + str(e) + "), using fallback")
                # Disable CUDA graphs permanently after failure
                self.use_cuda_graphs = False
        
        # Fallback path
        if not self.use_reduced_branching:
            print("Using standard GRU execution")
        
        if self.use_memory_optimization:
            # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Use pre-allocated h0
            (*@\greencode{h0 = self.h0.to(x.device)}@*)
        else:
            # Create new h0 each time
            h0 = self.h0.to(x.device).clone()
        
        # Use FP32 only - no mixed precision
        output, _ = self.gru(x, h0)
        return output

# Test code
batch_size = 10
seq_len = 512
input_size = 128
hidden_size = 256
num_layers = 6

def get_inputs():
    return [torch.randn(seq_len, batch_size, input_size)]

def get_init_inputs():
    return [input_size, hidden_size, num_layers]

# =============================================================================
# CONFIGURATION EXAMPLES
# =============================================================================
"""
(*@\emoji{control-knobs}@*) HOW TO USE THE 4 OPTIMIZATION SWITCHES:

1. Change the True/False values at the top of the file:
   USE_CUDA_GRAPHS = True/False        # Major speedup enabler
   USE_MEMORY_OPTIMIZATION = True/False # Moderate speedup + enables other opts
   USE_STREAM_MANAGEMENT = True/False  # Critical for unlocking CUDA graphs potential
   USE_REDUCED_BRANCHING = True/False  # Final performance multiplier

2. Based on your benchmark results, test these key combinations:

# Elite Performance (400x+):
USE_CUDA_GRAPHS = True
USE_MEMORY_OPTIMIZATION = True
USE_STREAM_MANAGEMENT = True  
USE_REDUCED_BRANCHING = True

# Plateau Performance (260x):
USE_CUDA_GRAPHS = True
USE_MEMORY_OPTIMIZATION = True
USE_STREAM_MANAGEMENT = True  
USE_REDUCED_BRANCHING = False

# Stagnation (2x):
USE_CUDA_GRAPHS = True
USE_MEMORY_OPTIMIZATION = True/False
USE_STREAM_MANAGEMENT = False  # Missing the key enabler!
USE_REDUCED_BRANCHING = True/False

# Baseline (1x):
USE_CUDA_GRAPHS = False  # No CUDA graphs = no speedup
others = any value

KEY INSIGHT: Stream Management is the critical enabler that transforms
CUDA graphs from 2x to 260x+ performance!
"""

if __name__ == "__main__":
    print("(*@\emoji{control-knobs}@*) Model with 4 optimizations (Kernel Warmup excluded)")
    print("\nCurrent configuration:")
    print("(*@\emoji{blue-circle}@*) CUDA Graphs:        " + ("(*@\emoji{check-mark-button}@*) ON" if USE_CUDA_GRAPHS else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{green-circle}@*) Memory Optimization: " + ("(*@\emoji{check-mark-button}@*) ON" if USE_MEMORY_OPTIMIZATION else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{yellow-circle}@*) Kernel Warmup:      (*@\emoji{cross-mark}@*) OFF (EXCLUDED)")
    print("(*@\emoji{purple-circle}@*) Stream Management:  " + ("(*@\emoji{check-mark-button}@*) ON" if USE_STREAM_MANAGEMENT else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{red-circle}@*) Reduced Branching:  " + ("(*@\emoji{check-mark-button}@*) ON" if USE_REDUCED_BRANCHING else "(*@\emoji{cross-mark}@*) OFF"))

\end{lstlisting}

\label{tab:cuda-rl-five-techs}
\end{tcolorbox}




==> tables/ablation_optim_case_3dconv.tex <==
%\begin{table}[htbp]
%  \centering
  %============================= Outer container (single prompt)
  %\begin{adjustbox}{margin=-0.2cm 0cm 0cm 0cm, scale=0.9}
\captionof{table}{Reference code and CUDA-L1 generation for Conv3D class}

\begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Conv3D | Reference Code - Simple baseline implementation},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
%\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries,]
import torch
import torch.nn as nn

class Model(nn.Module):
    """
    Performs a standard 3D convolution operation with asymmetric input and kernel sizes.
    
    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (tuple): Size of the convolution kernel in the form (kernel_size_d, kernel_size_h, kernel_size_w).
        stride (tuple, optional): Stride of the convolution in the form (stride_d, stride_h, stride_w). Defaults to (1, 1, 1).
        padding (tuple, optional): Padding applied to the input in the form (padding_d, padding_h, padding_w). Defaults to (0, 0, 0).
        dilation (tuple, optional): Spacing between kernel elements in the form (dilation_d, dilation_h, dilation_w). Defaults to (1, 1, 1).
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: tuple, 
                 stride: tuple = (1, 1, 1), padding: tuple = (0, 0, 0), 
                 dilation: tuple = (1, 1, 1), groups: int = 1, bias: bool = False):
        super(Model, self).__init__()
        self.conv3d = nn.Conv3d(in_channels, out_channels, kernel_size, 
                                stride=stride, padding=padding, 
                                dilation=dilation, groups=groups, bias=bias)
        
    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D convolution.
        
        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).
        
        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        return self.conv3d(x)

# Test code
batch_size = 16
in_channels = 3
out_channels = 64
kernel_size = (3, 5, 7)  # Asymmetric kernel size
depth = 16
height = 256
width = 256

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size]  # Provide in_channels, out_channels, kernel_size for initialization

\end{lstlisting}
\label{tab:ablation-reference-code}
  \end{tcolorbox}


  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Conv3D | Fully Optimized Code - All optimizations enabled (x faster)},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries, stringstyle = \color{black},]
import torch
import torch.nn as nn
import torch.nn.functional as F
import math

# ===== OPTIMIZATION TOGGLE SWITCHES =====
# Top 3 CUDA optimization techniques for Conv3D
USE_CUDA_STREAMS = True        # (*@\emoji{blue-circle}@*) Tech 1: Dedicated CUDA streams (~124x speedup alone) 
USE_CUDNN_AUTOTUNING = True    # (*@\emoji{green-circle}@*) Tech 2: cuDNN algorithm selection (~1-2x additional) 
USE_TF32_ACCELERATION = True   # (*@\emoji{yellow-circle}@*) Tech 3: TensorFloat-32 acceleration (~1-2x additional) 
# =========================================

class OptimizedConv3d(nn.Module):
    def __init__(self, in_channels, out_channels, kernel_size, stride=(1, 1, 1), 
                 padding=(0, 0, 0), dilation=(1, 1, 1), groups=1, bias=False):
        super(OptimizedConv3d, self).__init__()
        
        # Convert scalar values to tuples if needed
        if isinstance(kernel_size, int):
            kernel_size = (kernel_size, kernel_size, kernel_size)
        if isinstance(stride, int):
            stride = (stride, stride, stride)
        if isinstance(padding, int):
            padding = (padding, padding, padding)
        if isinstance(dilation, int):
            dilation = (dilation, dilation, dilation)
            
        self.in_channels = in_channels
        self.out_channels = out_channels
        self.kernel_size = kernel_size
        self.stride = stride
        self.padding = padding
        self.dilation = dilation
        self.groups = groups
        
        # Initialize weights
        self.weight = nn.Parameter(torch.empty(out_channels, in_channels // groups, *kernel_size))
        nn.init.kaiming_uniform_(self.weight, a=math.sqrt(5))
        
        if bias:
            self.bias = nn.Parameter(torch.empty(out_channels))
            fan_in, _ = nn.init._calculate_fan_in_and_fan_out(self.weight)
            bound = 1 / math.sqrt(fan_in)
            nn.init.uniform_(self.bias, -bound, bound)
        else:
            self.register_parameter('bias', None)
        
        # (*@\emoji{green-circle}@*) Tech 2: Enable cuDNN optimizations
        if torch.cuda.is_available() and USE_CUDNN_AUTOTUNING:
            (*@\greencode{torch.backends.cudnn.benchmark = True}@*)
            (*@\greencode{torch.backends.cudnn.deterministic = False}@*)
            
        # (*@\emoji{yellow-circle}@*) Tech 3: Enable TF32 acceleration
        if torch.cuda.is_available() and USE_TF32_ACCELERATION:
            (*@\yellowcode{if hasattr(torch.backends.cudnn, 'allow\_tf32'):}@*)
                (*@\yellowcode{torch.backends.cudnn.allow\_tf32 = True}@*)
            (*@\yellowcode{if hasattr(torch, 'set\_float32\_matmul\_precision'):}@*)
                (*@\yellowcode{torch.set\_float32\_matmul\_precision('high')}@*)
        
        # (*@\emoji{blue-circle}@*) Tech 1: Create a dedicated CUDA stream
        (*@\bluecode{self.stream = torch.cuda.Stream() if (torch.cuda.is\_available() and USE\_CUDA\_STREAMS) else None}@*)
        
        # State tracking
        self.initialized = False
        self.weight_device = None
    
    def _ensure_weight_on_device(self, device):
        """Ensure weights are on the correct device"""
        if self.weight.device != device or self.weight_device != device:
            self.weight.data = self.weight.data.to(device)
            if self.bias is not None:
                self.bias.data = self.bias.data.to(device)
            self.weight_device = device
            
            # Warm up on first use
            if not self.initialized and device.type == 'cuda':
                dummy_input = torch.zeros(1, self.in_channels, 4, 4, 4, device=device)
                with torch.no_grad():
                    _ = F.conv3d(dummy_input, self.weight, self.bias, self.stride,
                                self.padding, self.dilation, self.groups)
                if device.type == 'cuda':
                    torch.cuda.synchronize()
                self.initialized = True
    
    def forward(self, x):
        # Ensure weights are on the same device as input
        self._ensure_weight_on_device(x.device)
        
        # (*@\emoji{blue-circle}@*) Tech 1: Use CUDA stream if available
        if USE_CUDA_STREAMS and self.stream is not None and x.is_cuda:
            (*@\bluecode{with torch.cuda.stream(self.stream):}@*)
                (*@\bluecode{output = F.conv3d(x, self.weight, self.bias, self.stride,}@*)
                                 (*@\bluecode{self.padding, self.dilation, self.groups)}@*)
        else:
            output = F.conv3d(x, self.weight, self.bias, self.stride,
                             self.padding, self.dilation, self.groups)
        
        return output

class ModelNew(nn.Module):
    """
    Performs a standard 3D convolution operation with asymmetric input and kernel sizes.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: tuple, 
                 stride: tuple = (1, 1, 1), padding: tuple = (0, 0, 0), 
                 dilation: tuple = (1, 1, 1), groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        self.conv3d = OptimizedConv3d(in_channels, out_channels, kernel_size, 
                                     stride=stride, padding=padding, 
                                     dilation=dilation, groups=groups, bias=bias)
        
    def forward(self, x: torch.Tensor) -> torch.Tensor:
        return self.conv3d(x)

\end{lstlisting}

\label{tab:conv3d-five-techs}
\end{tcolorbox}




==> tables/ablation_optim_case_v2.tex <==
\begin{table}[htbp]
%  \centering
  %============================= Outer container (single prompt)
  %\begin{adjustbox}{margin=-0.2cm 0cm 0cm 0cm, scale=0.9}
\newcommand{\bluecode}[1]{\textcolor{code-highlight-blue}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\greencode}[1]{\textcolor{code-highlight-green}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\yellowcode}[1]{\textcolor{code-highlight-yellow}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\purplecode}[1]{\textcolor{code-highlight-purple}{\bfseries\footnotesize\ttfamily #1}}
\newcommand{\redcode}[1]{\textcolor{code-highlight-red}{\bfseries\footnotesize\ttfamily #1}}

\captionof{table}{Reference code and CUDA-L1 generation for Bidirectional GRU class}
  
  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Bidirectional GRU | Reference Code - Simple baseline implementation},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries,]
class ModelReference(nn.Module):
    def __init__(self, input_size, hidden_size, num_layers=3, bias=True, batch_first=False):
        """
        Simple reference implementation - no optimizations
        """
        super(ModelReference, self).__init__()
        
        self.gru = nn.GRU(input_size, hidden_size, num_layers, }bias, batch_first, dropout=0, bidirectional=True)
        self.h0 = torch.randn((num_layers * 2, 10, hidden_size))  # batch_size=10
    
    def forward(self, x):
        """
        Basic forward pass with no optimizations
        """
        self.h0 = self.h0.to(x.device)
        output, h_n = self.gru(x, self.h0)
        return output

\end{lstlisting}
\label{tab:ablation-reference-code}
  \end{tcolorbox}


  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    enlarge left by=-1cm,
    width=1.1\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{ Bidirectional GRU | Fully Optimized Code - All optimizations enabled (400x faster)},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=-1pt,
    right=2pt,
    top=2pt,
    bottom=2pt
  ]
\vspace{-0.05cm}
%normalsize
\begin{lstlisting}[language=Python, style=py, basicstyle=\footnotesize\ttfamily, frame=none,framerule=0pt, escapeinside={(*@}{@*)}, backgroundcolor=\color{gray!5}, keywordstyle = \color{templateblue}\bfseries, stringstyle = \color{black},]
import torch
import torch.nn as nn

# (*@\emoji{control-knobs}@*) ========== OPTIMIZATION TOGGLE SWITCHES ==========
# Change these True/False values to enable/disable optimizations
USE_CUDA_GRAPHS = True         # (*@\emoji{blue-circle}@*) CUDA graph capture and replay
USE_MEMORY_OPTIMIZATION = True # (*@\emoji{green-circle}@*) Pre-allocation and caching  
USE_STREAM_MANAGEMENT = True   # (*@\emoji{purple-circle}@*) Dedicated CUDA streams
USE_REDUCED_BRANCHING = True   # (*@\emoji{red-circle}@*) Minimal conditional logic

# (*@\emoji{cross-mark}@*) KERNEL WARMUP is EXCLUDED from this model
# =====================================================

class ModelNew(nn.Module):
    def __init__(self, input_size, hidden_size, num_layers=3, bias=True, batch_first=False):
        """
        Model with 4 optimizations (excluding kernel warmup)
        
        Edit the USE_* variables above to enable/disable optimizations
        """
        super(ModelNew, self).__init__()
        
        self.gru = nn.GRU(input_size, hidden_size, num_layers, bias, batch_first, 
                          dropout=0, bidirectional=True)
        
        # (*@\emoji{control-knobs}@*) OPTIMIZATION SWITCHES (from global variables)
        self.use_cuda_graphs = USE_CUDA_GRAPHS
        self.use_memory_optimization = USE_MEMORY_OPTIMIZATION
        self.use_stream_management = USE_STREAM_MANAGEMENT
        self.use_reduced_branching = USE_REDUCED_BRANCHING
        
        # Always have the base hidden state
        self.h0 = torch.randn((num_layers * 2, 10, hidden_size))  # batch_size=10
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS variables (always initialized for consistency)
        self.graph = None
        self.static_input = None
        self.static_h0 = None
        self.static_output = None
        self.static_hn = None
        self.expected_shape = None
        self.expected_device = None
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION variables
        self.graph_cache = {} if self.use_memory_optimization else None
        
        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT variables
        self.stream = None
        
        # (*@\emoji{red-circle}@*) REDUCED BRANCHING variables
        self.call_count = 0
        
        # Print configuration
        self._print_config()
    
    def _print_config(self):
        """Print current optimization configuration"""
        print("(*@\emoji{control-knobs}@*)  OPTIMIZATION CONFIGURATION:")
        print("(*@\emoji{blue-circle}@*) CUDA Graphs: " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_cuda_graphs else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{green-circle}@*) Memory Optimization: " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_memory_optimization else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{yellow-circle}@*) Kernel Warmup:   (*@\emoji{cross-mark}@*) OFF (EXCLUDED)")
        print("(*@\emoji{purple-circle}@*) Stream Management:  " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_stream_management else "(*@\emoji{cross-mark}@*) OFF"))
        print("(*@\emoji{red-circle}@*) Reduced Branching:  " + ("(*@\emoji{check-mark-button}@*) ON " if self.use_reduced_branching else "(*@\emoji{cross-mark}@*) OFF"))
        print("=" * 50)
    
    def _get_graph_key(self, x):
        """(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Generate unique key for graph caching (if enabled)"""
        if self.use_memory_optimization:
            (*@\greencode{return (x.shape, str(x.device))}@*)
        return None
    
    def _initialize_cuda_graph(self, x):
        """(*@\emoji{blue-circle}@*) CUDA GRAPHS: Initialize graph with conditional optimizations (no warmup)"""
        
        if not self.use_reduced_branching:
            print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Initializing CUDA graph...")
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Check cache first (if enabled)
        if self.use_memory_optimization:
            (*@\greencode{shape\_key = self.\_get\_graph\_key(x)}@*)
            (*@\greencode{if shape\_key and shape\_key in self.graph\_cache:}@*)
                (*@\greencode{cached\_data = self.graph\_cache[shape\_key]}@*)
                (*@\greencode{self.graph = cached\_data['graph']}@*)
                (*@\greencode{self.static\_input = cached\_data['input']}@*)
                (*@\greencode{self.static\_output = cached\_data['output']}@*)
                (*@\greencode{self.static\_h0 = cached\_data['h0']}@*)
                (*@\greencode{self.static\_hn = cached\_data['hn']}@*)
                (*@\greencode{self.expected\_shape = x.shape}@*)
                (*@\greencode{self.expected\_device = x.device}@*)
                if not self.use_reduced_branching:
                    print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Using cached graph")
                return
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Store expected characteristics
        self.expected_shape = x.shape
        self.expected_device = x.device
        
        # Create static tensors
        self.static_input = torch.zeros_like(x, device=x.device)
        
        if self.use_memory_optimization:
            #(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Use pre-allocated h0
            (*@\greencode{self.static\_h0 = self.h0.to(x.device).contiguous()}@*)
        else:
            # Create new h0 each time (less efficient)
            h0 = self.h0.to(x.device).clone()
            self.static_h0 = h0.contiguous()
        
        # Determine output shape
        if self.gru.batch_first:
            batch_size, seq_len = x.shape[:2]
            output_shape = (batch_size, seq_len, self.gru.hidden_size * 2)
        else:
            seq_len, batch_size = x.shape[:2]
            output_shape = (seq_len, batch_size, self.gru.hidden_size * 2)
        
        self.static_output = torch.zeros(output_shape, device=x.device)
        self.static_hn = torch.zeros((self.gru.num_layers * 2, batch_size, self.gru.hidden_size), 
                                    device=x.device)
        
        # (*@\emoji{cross-mark}@*) NO KERNEL WARMUP: Skip warmup - kernels will compile during graph capture
        # This may cause slower first execution
        
        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Create dedicated stream (if enabled)
        if self.use_stream_management and self.stream is None:
            (*@\purplecode{self.stream = torch.cuda.Stream()}@*)
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Capture the computation graph
        self.static_input.copy_(x)

        # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Use dedicated stream
        if self.use_stream_management:
            (*@\purplecode{self.stream.wait\_stream(torch.cuda.current\_stream())}@*)
            (*@\purplecode{with torch.cuda.stream(self.stream):}@*)
                (*@\purplecode{self.graph = torch.cuda.CUDAGraph()}@*)
                (*@\purplecode{with torch.cuda.graph(self.graph):}@*)
                    # Use FP32 only - no mixed precision
                    (*@\purplecode{output, hn = self.gru(self.static\_input, self.static\_h0)}@*)
                    (*@\purplecode{self.static\_output.copy\_(output)}@*)
                    (*@\purplecode{self.static\_hn.copy\_(hn)}@*)
        else:
            # Use default stream
            self.graph = torch.cuda.CUDAGraph()
            with torch.cuda.graph(self.graph):
                # Use FP32 only - no mixed precision
                output, hn = self.gru(self.static_input, self.static_h0)
                self.static_output.copy_(output)
                self.static_hn.copy_(hn)
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Cache the graph (if enabled)
        if self.use_memory_optimization and shape_key:
            (*@\greencode{self.graph\_cache[shape\_key] = \{}@*)
                (*@\greencode{'graph': self.graph,}@*)
                (*@\greencode{'input': self.static\_input,}@*)
                (*@\greencode{'output': self.static\_output,}@*)
                (*@\greencode{'h0': self.static\_h0,}@*)
                (*@\greencode{'hn': self.static\_hn}@*)
            (*@\greencode{\}}@*)
            if not self.use_reduced_branching:
                print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Cached graph for shape " + str(x.shape))
    
    def forward(self, x):
        """
        Forward pass with configurable optimizations (no kernel warmup)
        """
        
        # (*@\emoji{red-circle}@*) REDUCED BRANCHING: Conditional debugging
        if not self.use_reduced_branching:
            (*@\redcode{self.call\_count += 1}@*)
            print("\n--- Forward pass #" + str(self.call_count) + " ---")
            print("Input shape: " + str(x.shape) + ", device: " + str(x.device))
        
        # Fast path for CPU
        if not x.is_cuda:
            h0 = self.h0.to(x.device)
            # Use FP32 only - no mixed precision
            output, _ = self.gru(x, h0)
            return output
        
        # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Contiguous check (if enabled)
        if self.use_memory_optimization and not x.is_contiguous():
            (*@\greencode{x = x.contiguous()}@*)
            if not self.use_reduced_branching:
                print("(*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Made input contiguous")
        
        # (*@\emoji{blue-circle}@*) CUDA GRAPHS: Try to use CUDA graphs (if enabled)
        if self.use_cuda_graphs:
            try:
                # Check if graph needs initialization
                (*@\bluecode{need\_init = (self.graph is None or }@*)
                           (*@\bluecode{self.expected\_shape != x.shape or}@*) 
                           (*@\bluecode{self.expected\_device != x.device)}@*) 
                
                (*@\bluecode{if need\_init:}@*)
                    (*@\bluecode{if not self.use\_reduced\_branching:}@*)
                        (*@\bluecode{print("\emoji{blue-circle} CUDA GRAPHS: Initializing graph")}@*)
                    (*@\bluecode{with torch.no\_grad():}@*)
                        (*@\bluecode{self.\_initialize\_cuda\_graph(x)}@*)
                
                # Execute with CUDA graph
                (*@\bluecode{self.static\_input.copy\_(x)}@*)
                
                if self.use_stream_management:
                    # (*@\emoji{purple-circle}@*) STREAM MANAGEMENT: Execute in dedicated stream
                    (*@\purplecode{with torch.cuda.stream(self.stream):}@*)
                        (*@\purplecode{self.graph.replay()}@*)
                else:
                    # Execute on default stream
                    self.graph.replay()
                
                if not self.use_reduced_branching:
                    print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Graph executed successfully")
                
                return self.static_output
                
            except Exception as e:
                if not self.use_reduced_branching:
                    print("(*@\emoji{blue-circle}@*) CUDA GRAPHS: Failed (" + str(e) + "), using fallback")
                # Disable CUDA graphs permanently after failure
                self.use_cuda_graphs = False
        
        # Fallback path
        if not self.use_reduced_branching:
            print("Using standard GRU execution")
        
        if self.use_memory_optimization:
            # (*@\emoji{green-circle}@*) MEMORY OPTIMIZATION: Use pre-allocated h0
            (*@\greencode{h0 = self.h0.to(x.device)}@*)
        else:
            # Create new h0 each time
            h0 = self.h0.to(x.device).clone()
        
        # Use FP32 only - no mixed precision
        output, _ = self.gru(x, h0)
        return output

# Test code
batch_size = 10
seq_len = 512
input_size = 128
hidden_size = 256
num_layers = 6

def get_inputs():
    return [torch.randn(seq_len, batch_size, input_size)]

def get_init_inputs():
    return [input_size, hidden_size, num_layers]

==============================================================================
       (*@\emoji{control-knobs}@*)  FOUR PERFORMANCE TOGGLES   (*@\emoji{control-knobs}@*)
==============================================================================
"""
There are four Boolean flags at the top of this file.  Toggle them to dial in
the exact balance between raw speed, memory use, and code complexity.

--- Flag ----------------------------------------------------------------------
│ USE_CUDA_GRAPHS             │ The heavy hitter.  When True you unlock the   │
│                             │ CUDA graph engine and open the door to        │
│                             │ hundred-fold speed-ups.                       │
-------------------------------------------------------------------------------
│ USE_MEMORY_OPTIMIZATION     │ Buffer re-use & kernel fusion.  Grants a      │
│                             │ moderate boost on its own and is a            │
│                             │ prerequisite for several other tweaks.        │
-------------------------------------------------------------------------------
│ USE_STREAM_MANAGEMENT       │ Assigns work to dedicated CUDA streams.       │
│                             │ This is the “secret sauce” that lets graphs   │
│                             │ scale from 2× to 250×+.                       │
-------------------------------------------------------------------------------
│ USE_REDUCED_BRANCHING       │ Removes divergent code paths.  Finishing      │
│                             │ touch that can multiply whatever gains you    │
│                             │ already have.                                 │
-------------------------------------------------------------------------------


PRE-BUILT PROFILES
------------------------
Toggle the flags as shown below to reproduce common performance tiers.

Profile Name        CG   MEM  STM  BR   Expected Speed-up
-----------------------------------------------------------------
ELITE               T    T    T    T    ≈ 400× or higher
PLATEAU             T    T    T    F    ≈ 260×
STAGNANT            T    *    F    *    ≈   2×   (* = either value)
BASELINE            F    *    *    *    ≈   1×

Key Take-Away
------------------------
Stream Management (STM) is the critical enabler.  
Without it, CUDA graphs plateau at ~2×; with it, they can rocket past 260×,
especially when all other switches are also enabled.
"""

if __name__ == "__main__":
    print("(*@\emoji{control-knobs}@*) Model with 4 optimizations (Kernel Warmup excluded)")
    print("\nCurrent configuration:")
    print("(*@\emoji{blue-circle}@*) CUDA Graphs:        " + ("(*@\emoji{check-mark-button}@*) ON" if USE_CUDA_GRAPHS else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{green-circle}@*) Memory Optimization: " + ("(*@\emoji{check-mark-button}@*) ON" if USE_MEMORY_OPTIMIZATION else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{yellow-circle}@*) Kernel Warmup:      (*@\emoji{cross-mark}@*) OFF (EXCLUDED)")
    print("(*@\emoji{purple-circle}@*) Stream Management:  " + ("(*@\emoji{check-mark-button}@*) ON" if USE_STREAM_MANAGEMENT else "(*@\emoji{cross-mark}@*) OFF"))
    print("(*@\emoji{red-circle}@*) Reduced Branching:  " + ("(*@\emoji{check-mark-button}@*) ON" if USE_REDUCED_BRANCHING else "(*@\emoji{cross-mark}@*) OFF"))

\end{lstlisting}

\label{tab:cuda-rl-five-techs}
\end{tcolorbox}


==> tables/ablation_optim_setup_and_results.tex <==
\begin{table*}[!ht]
\centering
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{adjustbox}{margin=-0.8cm 0cm 0cm 0cm, scale=1.0}
%\setlength{\tabcolsep}{8pt} 
\renewcommand\arraystretch{1.2}      % ① 行距放大
\setlength{\extrarowheight}{4pt}      % ② 每行额外+2pt
\begin{tabular}{C{2.2cm}C{2.2cm}C{2.2cm}C{2.8cm}|C{3.2cm}}
\toprule
{\small Cuda Graphs}  &  {\small Memory Optim}  & {\small Stream Manage} & {\small Reduced Branching} & \multirow{2}{*}{{\bf Speedup}} \\ 

{\small \emoji{blue-circle}} & {\small \emoji{green-circle}} & {\small \emoji{purple-circle}} & {\small \emoji{red-circle}} &  \\\midrule

%%%%%%%%%%%%%%%%
% 1 2 4 5 
\emoji{check-mark}     &    \emoji{check-mark}    & \emoji{check-mark}  & \emoji{check-mark} & {\bf 446.2x}~\emoji{rocket} \\

%%%%%%%%%%%%
% 1 4 5
\emoji{check-mark} & \emoji{cross-mark}& \emoji{check-mark}& \emoji{check-mark} & {\bf 405.2x}~\emoji{rocket} \\

%%%%%%%%%%%%
% 1 2 3 4 
\emoji{check-mark} & \emoji{check-mark}& \emoji{check-mark}& \emoji{cross-mark} & {\bf  268.6x}~\emoji{rocket}\\

%%%%%%%%%%%%
% 1  3 4  
\emoji{check-mark} &  \emoji{cross-mark} & \emoji{check-mark}&  \emoji{cross-mark}& {\bf  262.1x}~\emoji{rocket} \\

%%%%%%%%%%%%
% 1 5
\emoji{check-mark} &  \emoji{cross-mark} & \emoji{cross-mark} &  \emoji{check-mark} &  2.0x \\

%%%%%%%%%%%%
% 1 2 3 5
\emoji{check-mark} &  \emoji{check-mark} & \emoji{cross-mark} &  \emoji{check-mark} &   2.0x  \\

%%%%%%%%%%%%
% 1 2 3 
\emoji{check-mark} &  \emoji{check-mark} & \emoji{cross-mark} &  \emoji{cross-mark} &  2.0x   \\

%%%%%%%%%%%%
% 1 3 
\emoji{check-mark} & \emoji{cross-mark} & \emoji{cross-mark} & \emoji{cross-mark} &  2.0x \\

%%%%%%%%%%%%
% 2 5
\emoji{cross-mark} & \emoji{check-mark} & \emoji{cross-mark} & \emoji{check-mark} &      1.0x   \\

%%%%%%%%%%%%
% 3 5
\emoji{cross-mark} & \emoji{cross-mark} & \emoji{cross-mark} & \emoji{check-mark} &    1.0x   \\

%%%%%%%%%%%%
% 2 3 
\emoji{cross-mark} & \emoji{check-mark} & \emoji{cross-mark} & \emoji{cross-mark} &      1.0x     \\

%%%%%%%%%%%%
% 2 3 4 5
\emoji{cross-mark} &\emoji{check-mark} & \emoji{check-mark}  & \emoji{check-mark} &     1.0x    \\

%%%%%%%%%%%%
% 3 4 5
\emoji{cross-mark} &\emoji{cross-mark} & \emoji{check-mark}  & \emoji{check-mark} &    1.0x     \\

%%%%%%%%%%%%
% 4 5
\emoji{cross-mark} &\emoji{cross-mark} & \emoji{check-mark}  & \emoji{cross-mark} & 1.0x \\

%%%%%%%%%%%%
% 2 4
\emoji{cross-mark} & \emoji{check-mark} & \emoji{check-mark}  & \emoji{cross-mark} &1.0x  \\

%%%%%%%%%%%%
% 3
\emoji{cross-mark} & \emoji{cross-mark} & \emoji{cross-mark} & \emoji{cross-mark} & 1.0x \\

\bottomrule
 \end{tabular}
 \end{adjustbox}
\caption{Configs used in Section xxxxx experiment.}
\label{all-level-results}
\end{table*}

==> tables/ablation_optim_type.tex <==
%\clearpage 
\newpage
\newgeometry{margin=1cm, height=70cm} 

\begin{table*}[p]
%\vspace{-15cm}
\centering
\small
\begin{adjustbox}{margin=-1.5cm 0cm 0cm 0cm, scale=0.7}
\begin{tabular}{
p{5cm}
@{\hspace{1cm}} 
>{\columncolor{refgreen!10}}p{8cm}
@{\hspace{0.6cm}} 
>{\columncolor{refgreen!10}}p{8cm}
p{2cm}
}
\toprule
\color{black}{\bf Tech} & \multicolumn{2}{l}{\cellcolor{white} \color{black}{\bf Implementation}} & \cellcolor{white} {\bf \color{black}{Score}} \\
\midrule
\begin{minipage}[t]{\linewidth}
\textbf{CUDA-L1 Output (400x faster)} \\ 

All optimizations enabled:
\begin{itemize}
    \item w/ CUDA Graphs
    \item w/ Memory Optimization
    \item w/ Kernel Warmup
    \item w/ Stream Management
    \item w/ Stream Management
    \item w/ Reduced Branching
\end{itemize}
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\vspace{-0.4cm}
% {\bf \color{refgreen}{- Naive matrix multiplication with poor memory access}}
\begin{lstlisting}[style=beforeoptimcode, language = Python, escapeinside={<@}{@>}]
class ModelFullyOptimized(nn.Module):
    <@\textcolor{red}{def \_\_init\_\_(self, input\_size, hidden\_size, num\_layers=3, bias=True, batch\_first=False):}@>
        """
        Fully optimized implementation with all performance techniques
        """
        super(ModelFullyOptimized, self).__init__()
        
        # Create the GRU with the exact same parameters as reference
        self.gru = nn.GRU(input_size, hidden_size, num_layers, bias, batch_first, 
                          dropout=0, bidirectional=True)
        # Initialize hidden state (Memory Optimization)
        self.h0 = torch.randn((num_layers * 2, 10, hidden_size))  # batch_size=10
        # CUDA graph optimization
        self.graph = None
        self.static_input = None
        self.static_h0 = None
        self.static_output = None
        self.static_hn = None
        # Expected shape for CUDA graph
        self.expected_shape = None
        self.expected_device = None
        # Track whether we've done warmup (Kernel Warmup)
        self.warmed_up = False
        # Stream for graph execution (Stream Management)
        self.stream = None
        # Graph cache by input shape and device (Memory Optimization)
        self.graph_cache = {}
        # Flag to indicate if we're using CUDA graphs
        self.use_cuda_graphs = True
    
    def _warmup(self, x, h0):
        """Perform warmup runs to ensure kernels are compiled (Kernel Warmup)"""
        if not self.warmed_up and x.is_cuda:
            with torch.no_grad():
                for _ in range(3):
                    _ = self.gru(x, h0)
            self.warmed_up = True

    def _get_graph_key(self, x):
        """Generate a unique key for graph caching (Memory Optimization)"""
        return (x.shape, str(x.device))
    
    def _initialize_cuda_graph(self, x):
        """Initialize CUDA graph for the given input shape (CUDA Graphs)"""
        # Create a shape key for caching
        shape_key = self._get_graph_key(x)
        # Check if we have a cached graph for this shape and device
        if shape_key in self.graph_cache:
            cached_data = self.graph_cache[shape_key]
            self.graph = cached_data['graph']
            self.static_input = cached_data['input']
            self.static_output = cached_data['output']
            self.static_h0 = cached_data['h0']
            self.static_hn = cached_data['hn']
            self.expected_shape = x.shape
            self.expected_device = x.device
            return
        # Store expected shape and device
        self.expected_shape = x.shape
        self.expected_device = x.device
        # Create static tensors for graph capture (Memory Optimization)
        self.static_input = torch.zeros_like(x, device=x.device)
        self.static_h0 = self.h0.to(x.device).contiguous()
        # Determine output shape
        if self.gru.batch_first:
            batch_size, seq_len = x.shape[:2]
            output_shape = (batch_size, seq_len, self.gru.hidden_size * 2)
        else:
            seq_len, batch_size = x.shape[:2]
            output_shape = (seq_len, batch_size, self.gru.hidden_size * 2)
            
        self.static_output = torch.zeros(output_shape, device=x.device)
        self.static_hn = torch.zeros((self.gru.num_layers * 2, batch_size, self.gru.hidden_size), 
                                    device=x.device)
\end{lstlisting} 
\end{minipage} 
& 
\begin{minipage}[t]{\linewidth}
\vspace{-0.4cm}
% {\bf \color{refgreen}{- Naive matrix multiplication with poor memory access}}
\begin{lstlisting}[style=beforeoptimcode, language = Python, firstnumber=75]
        # Warmup runs to ensure kernels are compiled (Kernel Warmup)
        self._warmup(x, self.static_h0)
        # Create a dedicated stream for graph execution (Stream Management)
        if self.stream is None:
            self.stream = torch.cuda.Stream()
        # Capture the graph (CUDA Graphs)
        self.static_input.copy_(x)
        self.stream.wait_stream(torch.cuda.current_stream())
        
        with torch.cuda.stream(self.stream):
            self.graph = torch.cuda.CUDAGraph()
            with torch.cuda.graph(self.graph):
                with amp.autocast(enabled=True):
                    output, hn = self.gru(self.static_input, self.static_h0)
                self.static_output.copy_(output)
                self.static_hn.copy_(hn)
        
        # Cache the graph and associated tensors (Memory Optimization)
        self.graph_cache[shape_key] = {
            'graph': self.graph,
            'input': self.static_input,
            'output': self.static_output,
            'h0': self.static_h0,
            'hn': self.static_hn
        }
        
    def forward(self, x):
        """
        Optimized forward pass with minimal branching (Reduced Branching)
        """
        # Fast path for non-CUDA tensors
        if not x.is_cuda:
            h0 = self.h0.to(x.device)
            with amp.autocast(enabled=True):
                output, _ = self.gru(x, h0)
            return output
        # Ensure input is contiguous for better memory access (Memory Optimization)
        if not x.is_contiguous():
            x = x.contiguous()
        # Try to use CUDA graphs for optimization (CUDA Graphs)
        if self.use_cuda_graphs:
            try:
                # Check if we need to initialize or reinitialize the CUDA graph
                shape_changed = self.expected_shape != x.shape
                device_changed = self.expected_device != x.device
                
                if self.graph is None or shape_changed or device_changed:
                    with torch.no_grad():
                        self._initialize_cuda_graph(x)
                
                # Run with CUDA graph - minimal branching in hot path (Reduced Branching)
                self.static_input.copy_(x)
                
                with torch.cuda.stream(self.stream):  # Stream Management
                    self.graph.replay()  # CUDA Graphs
                
                # No need to wait for the stream if we're just returning the output
                # The next CUDA operation will implicitly synchronize
                return self.static_output
                
            except Exception:
                # Fall back to regular execution if CUDA graph fails
                self.use_cuda_graphs = False
        
        # Fallback path if CUDA graphs are disabled or failed
        h0 = self.h0.to(x.device)
        with amp.autocast(enabled=True):
            output, _ = self.gru(x, h0)
        return output
\end{lstlisting} 
\end{minipage}  & 
\color{red}{na score} \\\midrule

\begin{comment}
CUDA-L1 & 
\begin{minipage}[t]{\linewidth}
\vspace{-0.4cm}
% {\bf \color{refgreen}{- Naive matrix multiplication with poor memory access}}
\begin{lstlisting}[style=beforeoptimcode, language = Python, ]

    def _get_graph_key(self, x):
        """Generate a unique key for graph caching (Memory Optimization)"""
        return (x.shape, str(x.device))
    
    def _initialize_cuda_graph(self, x):
        """Initialize CUDA graph for the given input shape (CUDA Graphs)"""
        # Create a shape key for caching
        shape_key = self._get_graph_key(x)
        # Check if we have a cached graph for this shape and device
        if shape_key in self.graph_cache:
            cached_data = self.graph_cache[shape_key]
            self.graph = cached_data['graph']
            self.static_input = cached_data['input']
            self.static_output = cached_data['output']
            self.static_h0 = cached_data['h0']
            self.static_hn = cached_data['hn']
            self.expected_shape = x.shape
            self.expected_device = x.device
            return
        # Store expected shape and device
        self.expected_shape = x.shape
        self.expected_device = x.device
        # Create static tensors for graph capture (Memory Optimization)
        self.static_input = torch.zeros_like(x, device=x.device)
        self.static_h0 = self.h0.to(x.device).contiguous()
        # Determine output shape
        if self.gru.batch_first:
            batch_size, seq_len = x.shape[:2]
            output_shape = (batch_size, seq_len, self.gru.hidden_size * 2)
        else:
            seq_len, batch_size = x.shape[:2]
            output_shape = (seq_len, batch_size, self.gru.hidden_size * 2)
            
        self.static_output = torch.zeros(output_shape, device=x.device)
        self.static_hn = torch.zeros((self.gru.num_layers * 2, batch_size, self.gru.hidden_size), 
                                    device=x.device)
        # Warmup runs to ensure kernels are compiled (Kernel Warmup)
        self._warmup(x, self.static_h0)
        # Create a dedicated stream for graph execution (Stream Management)
        if self.stream is None:
            self.stream = torch.cuda.Stream()
        # Capture the graph (CUDA Graphs)
        self.static_input.copy_(x)
        self.stream.wait_stream(torch.cuda.current_stream())
        
        with torch.cuda.stream(self.stream):
            self.graph = torch.cuda.CUDAGraph()
            with torch.cuda.graph(self.graph):
                with amp.autocast(enabled=True):
                    output, hn = self.gru(self.static_input, self.static_h0)
                self.static_output.copy_(output)
                self.static_hn.copy_(hn)
        
        # Cache the graph and associated tensors (Memory Optimization)
        self.graph_cache[shape_key] = {
            'graph': self.graph,
            'input': self.static_input,
            'output': self.static_output,
            'h0': self.static_h0,
            'hn': self.static_hn
        }
    
    def forward(self, x):
        """
        Optimized forward pass with minimal branching (Reduced Branching)
        """
        # Fast path for non-CUDA tensors
        if not x.is_cuda:
            h0 = self.h0.to(x.device)
            with amp.autocast(enabled=True):
                output, _ = self.gru(x, h0)
            return output
        # Ensure input is contiguous for better memory access (Memory Optimization)
        if not x.is_contiguous():
            x = x.contiguous()
        # Try to use CUDA graphs for optimization (CUDA Graphs)
        if self.use_cuda_graphs:
            try:
                # Check if we need to initialize or reinitialize the CUDA graph
                shape_changed = self.expected_shape != x.shape
                device_changed = self.expected_device != x.device
                
                if self.graph is None or shape_changed or device_changed:
                    with torch.no_grad():
                        self._initialize_cuda_graph(x)
                
                # Run with CUDA graph - minimal branching in hot path (Reduced Branching)
                self.static_input.copy_(x)
                
                with torch.cuda.stream(self.stream):  # Stream Management
                    self.graph.replay()  # CUDA Graphs
                
                # No need to wait for the stream if we're just returning the output
                # The next CUDA operation will implicitly synchronize
                return self.static_output
                
            except Exception:
                # Fall back to regular execution if CUDA graph fails
                self.use_cuda_graphs = False
        
        # Fallback path if CUDA graphs are disabled or failed
        h0 = self.h0.to(x.device)
        with amp.autocast(enabled=True):
            output, _ = self.gru(x, h0)
        return output
\end{lstlisting} 
\end{minipage} 
& 
\color{red}{na score} \\\midrule
\end{comment}

\end{tabular}
\end{adjustbox}
\caption{Ablation Study}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\restoregeometry  % 恢复原始设置
\newpage

==> tables/ablation_step3k_case.tex <==
% —— 前置：确保预先已 \usepackage{tcolorbox, listings, xcolor} 且定义了 templateblue ——
%\begin{table}

  % ============================= Outer container (single code example)
  \begin{tcolorbox}[
    rounded corners,
    enhanced jigsaw,
  breakable,
  colframe=templateblue,
  colback=white,
  title=\textbf{When $step = 3,000$, Model Generation ($score = 1.37$)},
  fonttitle=\bfseries,
  width=0.96\textwidth,
  boxrule=0.6pt,
  left=2pt, right=2pt, top=1pt, bottom=1pt,
  listing only,
  listing options={style=py, frame=none, breaklines=true}

  ]

  \begin{tcolorbox}[
  sharp corners,
  colframe=analysisblue,
  colback=analysisblue!5,
  colbacktitle=analysisblue!15,
  coltitle=analysisblue,
  boxrule=0.4pt,
  title={\textbf{Analysis}},
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=4pt,
  breakable
]

Based on the previous attempts, we have functionally correct implementations. The scores for the successful attempts are around 1.27-1.28x speedup over the reference implementation. Let's analyze what happened: 
\begin{itemize}
    \item Attempt \#1 achieved the highest score (1.38), using specialized weight formats and memory layout optimizations
    \item Attempt \#2 failed with an error about output padding being too large, showing that parameter handling is critical
    \item  Attempts \#3 and \#4 were successful but slightly slower than \#1 (1.27x speedup)\\
\end{itemize}

The key insights from successful implementations: 

\begin{enumerate}
    \item {\bf Memory layout optimization} is crucial - using $channels\_last\_3d$ format and ensuring contiguity.
    \item {\bf Weight preprocessing} into specialized formats for grouped convolutions shows significant benefits.
    \item {\bf Parameter correctness} is critical - especially setting $output\_padding=0$ explicitly.
    \item {\bf Group-specific optimizations} are effective since we're dealing with $groups=4$. The biggest bottleneck in the reference implementation appears to be suboptimal memory access patterns for grouped convolutions. \\
\end{enumerate}


The reference implementation uses {\bf nn.ConvTranspose3d} directly, which may not be optimized for the specific group size and tensor dimensions we're working with. For our optimized implementation, I'll build on the successful approach from attempt \#1 (which had the highest score) while ensuring proper parameter handling and focusing on optimizing the memory layout for the grouped transposed convolution operation.
\end{tcolorbox}

%============================= Part Y: Algorithm Description Section
\begin{tcolorbox}[
  sharp corners,
    breakable,
  colframe=algoyellow,
  colback=algoyellow!5,
  colbacktitle=algoyellow!15,
  coltitle=algoyellow,
  boxrule=0.4pt,
  title={\textbf{Algorithm Description}},
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=0pt,
  %after skip=0pt 
]
My optimization strategy focuses on maximizing performance for the specific 3D transposed convolution with $groups=4$: 

\begin{enumerate}
    \item {\bf Direct Function Implementation}: - Use F.conv\_transpose3d directly to minimize overhead - Ensure correct parameter handling, especially output\_padding=0.
    \item {\bf Memory Layout Optimization}: 
    \begin{itemize}
        \item Pre-process weights into multiple optimized formats
        \item Use channels\_last\_3d memory format for modern GPU architectures
        \item Ensure all tensors are properly contiguous
    \end{itemize}
    
    \item {\bf Group Convolution Specialization}: 
    \begin{itemize}
        \item Implement specialized handling for exactly 4 groups 
        \item Reorganize weights for better memory access patterns 
        \item Create multiple optimized weight formats for different execution scenarios 
    \end{itemize}

    \item {\bf Dynamic Execution Path Selection}:
    \begin{itemize}
        \item Select the optimal execution path based on input tensor characteristics
        \item Choose the best weight format based on input properties
        \item Implement specialized paths for the exact dimensions in this problem 
    \end{itemize}

     \item {\bf Tensor Preparation Optimization}:
     \begin{itemize}
        \item Ensure proper contiguity for all tensors
        \item Minimize tensor copies and format conversions 
        \item Implement efficient batch processing for large inputs
    \end{itemize}
    
\end{enumerate}

The key insight is to leverage PyTorch's already optimized implementations while ensuring optimal tensor layouts and access patterns, particularly for grouped transposed convolutions with the specific parameters in this use case.

\end{tcolorbox}

\begin{tcolorbox}[
     % blanker,          % 不自动生成内边距与行
  %hbox,             % 使整个盒子成为单行水平盒
  sharp corners,
  colframe=refgreen,
  colback=refgreen!15,
  boxrule=0.4pt,
  fontupper=\bfseries\small,
  left=4pt,right=4pt,top=4pt,bottom=4pt,
    ]
    {\bf \color{refgreen}{Code:}}
\end{tcolorbox}

\vspace{-0.4cm}
% --------------- Part 2: Previous CUDA implement with scores
% ----------------- 代码本体：直接用 listings，行号已“嵌入背景”
\begin{lstlisting}[style=py, frame=none, breaklines=true, ] 
import torch
import torch.nn as nn
import torch.nn.functional as F

class ModelNew(nn.Module):
    """
    Performs a 3D transposed convolution operation with asymmetric input and square kernel.
    The input is padded before the convolution.

    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (int): Size of the square convolution kernel.
        stride (int, optional): Stride of the convolution. Defaults to 1.
        padding (int, optional): Padding applied to the input. Defaults to 0.
        output_padding (int, optional): Additional size added to output shape. Defaults to 0.
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: int, stride: int = 1, padding: int = 0, output_padding: int = 0, groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        
        # Create the standard ConvTranspose3d layer to get the weights
        self.conv_transpose3d = nn.ConvTranspose3d(
            in_channels, out_channels, 
            kernel_size=(kernel_size, kernel_size, kernel_size), 
            stride=stride, 
            padding=padding,
            output_padding=output_padding,
            groups=groups, 
            bias=bias
        )
        
        # Store parameters for our optimized implementation
        self.in_channels = in_channels
        self.out_channels = out_channels
        self.kernel_size = kernel_size
        self.stride = stride
        self.padding = padding
        self.output_padding = output_padding
        self.groups = groups
        
        # Pre-process weights for faster computation
        with torch.no_grad():
            # Create standard contiguous weight
            weight = self.conv_transpose3d.weight.detach()
            self.register_buffer('weight_contiguous', weight.contiguous())
            
            # Create channels_last weight if available
            if hasattr(torch, 'channels_last_3d'):
                self.register_buffer('weight_channels_last', 
                                   weight.to(memory_format=torch.channels_last_3d).contiguous())
            else:
                self.register_buffer('weight_channels_last', None)
            
            # Create specialized weight format for grouped convolution
            if groups > 1:
                # Reshape for better memory access patterns in grouped convolution
                channels_per_group = out_channels // groups
                in_channels_per_group = in_channels // groups
                
                # Reorganize weight tensor for better memory access in grouped convolution
                weight_grouped = weight.view(groups, channels_per_group, in_channels_per_group, 
                                          kernel_size, kernel_size, kernel_size)
                weight_grouped = weight_grouped.contiguous()
                weight_grouped = weight_grouped.view(out_channels, in_channels // groups, 
                                                 kernel_size, kernel_size, kernel_size)
                self.register_buffer('weight_grouped', weight_grouped.contiguous())
                
                # Additional optimization for exactly 4 groups (the specific case in this problem)
                if groups == 4:
                    # Further optimize for exactly 4 groups
                    weight_g4 = weight.clone()
                    # Reorganize for optimal memory access with 4 groups
                    weight_g4 = weight_g4.view(4, out_channels // 4, in_channels // 4, 
                                            kernel_size, kernel_size, kernel_size)
                    weight_g4 = weight_g4.permute(1, 0, 2, 3, 4, 5).contiguous()
                    weight_g4 = weight_g4.view(out_channels, in_channels // 4, 
                                            kernel_size, kernel_size, kernel_size)
                    self.register_buffer('weight_g4', weight_g4.contiguous())
                    
                    # Create a specialized weight format for the exact dimensions in this problem
                    if out_channels == 64 and in_channels == 32 and kernel_size == 3:
                        # Create an even more specialized format for this exact case
                        weight_specialized = weight.clone()
                        weight_specialized = weight_specialized.view(4, 16, 8, kernel_size, kernel_size, kernel_size)
                        # Optimize memory layout for better cache utilization
                        weight_specialized = weight_specialized.permute(0, 2, 1, 3, 4, 5).contiguous()
                        weight_specialized = weight_specialized.view(4, 8, 16, kernel_size, kernel_size, kernel_size)
                        weight_specialized = weight_specialized.permute(0, 2, 1, 3, 4, 5).contiguous()
                        weight_specialized = weight_specialized.view(out_channels, in_channels // 4, 
                                                                  kernel_size, kernel_size, kernel_size)
                        self.register_buffer('weight_specialized', weight_specialized.contiguous())
                        
                        # Create an additional optimized format specifically for stride=2
                        if stride == 2:
                            weight_stride2 = weight.clone()
                            # Reorganize for optimal memory access with stride=2
                            weight_stride2 = weight_stride2.view(4, 16, 8, kernel_size, kernel_size, kernel_size)
                            weight_stride2 = weight_stride2.permute(0, 1, 2, 3, 5, 4).contiguous()
                            weight_stride2 = weight_stride2.view(out_channels, in_channels // 4, 
                                                              kernel_size, kernel_size, kernel_size)
                            self.register_buffer('weight_stride2', weight_stride2.contiguous())
                        else:
                            self.register_buffer('weight_stride2', None)
                    else:
                        self.register_buffer('weight_specialized', None)
                        self.register_buffer('weight_stride2', None)
                else:
                    self.register_buffer('weight_g4', None)
                    self.register_buffer('weight_specialized', None)
                    self.register_buffer('weight_stride2', None)
            else:
                self.register_buffer('weight_grouped', None)
                self.register_buffer('weight_g4', None)
                self.register_buffer('weight_specialized', None)
                self.register_buffer('weight_stride2', None)
            
            # Process bias if present
            if bias:
                self.register_buffer('bias_optimized', 
                                   self.conv_transpose3d.bias.detach().contiguous())
            else:
                self.register_buffer('bias_optimized', None)

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D transposed convolution.

        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).

        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        # Fast path for CUDA tensors
        if x.is_cuda:
            # Choose the best weight format based on input and configuration
            if self.groups == 4:
                if (self.weight_stride2 is not None and self.stride == 2 and 
                    x.shape[1] == self.in_channels and x.shape[0] == 16):
                    # Use highly specialized format for stride=2 and batch_size=16
                    weight = self.weight_stride2
                    # Ensure input is contiguous
                    if not x.is_contiguous():
                        x = x.contiguous()
                elif self.weight_specialized is not None and x.shape[1] == self.in_channels:
                    # Use highly specialized format for the exact dimensions in this problem
                    weight = self.weight_specialized
                    # Ensure input is contiguous
                    if not x.is_contiguous():
                        x = x.contiguous()
                elif self.weight_g4 is not None:
                    # Use specialized format for exactly 4 groups
                    weight = self.weight_g4
                    # Ensure input is contiguous
                    if not x.is_contiguous():
                        x = x.contiguous()
                else:
                    # Fallback to grouped weights
                    weight = self.weight_grouped
                    # Ensure input is contiguous
                    if not x.is_contiguous():
                        x = x.contiguous()
            elif self.groups > 1 and self.weight_grouped is not None:
                # Use specialized grouped weights for other group sizes
                weight = self.weight_grouped
                # Ensure input is contiguous
                if not x.is_contiguous():
                    x = x.contiguous()
            elif hasattr(torch, 'channels_last_3d') and self.weight_channels_last is not None:
                # Check if input is already in channels_last format
                if x.is_contiguous(memory_format=torch.channels_last_3d):
                    # Both input and weight in channels_last format
                    weight = self.weight_channels_last
                else:
                    # Convert input to channels_last if beneficial
                    batch_size = x.shape[0]
                    if batch_size >= 8 and self.out_channels >= 32:
                        # Only convert for larger batches and channel counts where it's beneficial
                        x = x.to(memory_format=torch.channels_last_3d)
                        weight = self.weight_channels_last
                    else:
                        # For smaller sizes, standard contiguous format may be better
                        if not x.is_contiguous():
                            x = x.contiguous()
                        weight = self.weight_contiguous
            else:
                # Standard contiguous format
                if not x.is_contiguous():
                    x = x.contiguous()
                weight = self.weight_contiguous
            
            # Direct call to F.conv_transpose3d with minimal overhead
            return F.conv_transpose3d(
                x,
                weight,
                self.bias_optimized,
                stride=self.stride,
                padding=self.padding,
                output_padding=0,  # Explicitly set to 0 to avoid issues
                groups=self.groups
            )
        
        # Fallback to standard implementation for non-CUDA tensors
        return self.conv_transpose3d(x)

# Test code
batch_size = 16
in_channels = 32
out_channels = 64
kernel_size = 3
depth = 16
height = 32
width = 32
stride = 2
padding = 3
groups = 4

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size, stride, padding, 0, groups]
\end{lstlisting}
\end{tcolorbox}

%\end{longtable}
%\end{table}
%\end{tcolorbox}
\captionof{table}{When $step = 3,000$, model generation result. And score of the code equals to 1.37.}

==> tables/ablation_step6k_case.tex <==
% —— 前置：确保预先已 \usepackage{tcolorbox, listings, xcolor} 且定义了 templateblue ——
%\begin{table}
\vspace{-7em}
\centering
  % ============================= Outer container (single code example)
  \begin{tcolorbox}[
    rounded corners,
    enhanced jigsaw,
  breakable,
  colframe=templateblue,
  colback=white,
  title=\textbf{When $step = 6,000$, Model Generation ($score = 7.16$)},
  fonttitle=\bfseries,
  width=0.96\textwidth,
  boxrule=0.6pt,
  left=2pt, right=2pt, top=1pt, bottom=1pt,
  listing only,
  listing options={style=py, frame=none, breaklines=true}

  ]

  \begin{tcolorbox}[
  sharp corners,
  colframe=analysisblue,
  colback=analysisblue!5,
  colbacktitle=analysisblue!15,
  coltitle=analysisblue,
  boxrule=0.4pt,
  title={\textbf{Analysis}},
  %fonttitle=\bfseries,
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=4pt
]

Looking at the performance patterns: 

\begin{itemize}
    \item All successful implementations use direct `F.conv\_transpose3d` calls instead of the PyTorch module, which reduces overhead. 
    \item Memory format optimization using `channels\_last\_3d` format appears to be beneficial, as it's used in all high-performing implementations.
    \item Weight pre-computation and storage in optimized formats during initialization is a common technique in the successful attempts. 
    \item CUDA streams are used to improve parallelism without explicit synchronization.
    \item cuDNN optimizations like enabling benchmarking and TF32 precision are consistently applied. 
\end{itemize}

The key differences between the implementations: 
\begin{itemize}
    \item No3 (6.23 score) has a cleaner implementation with appropriate weight format selection based on input characteristics.
    \item No1 (6.05 score) has similar optimizations but with slightly more complex weight handling. 
    \item No2 (5.58 score) adds more complex weight format optimizations but might have introduced some overhead.
    \item No4 (5.32 score) simplified the approach but lost some performance. 
\end{itemize} 

The biggest opportunities for improvement appear to be: 

\begin{itemize}
    \item Optimizing the weight format selection strategy based on input characteristics
    \item Efficient handling of grouped convolutions (as $groups=4$ in this case)
    \item Smart memory format conversion that avoids unnecessary operations
    \item Proper cuDNN configuration to leverage hardware acceleration \\
\end{itemize}

For our implementation, I'll combine the best elements from the successful attempts while avoiding unnecessary complexity that might introduce overhead.

\end{tcolorbox}

\vspace{-1em}

%============================= Part Y: Algorithm Description Section
\begin{tcolorbox}[
  sharp corners,
  colframe=algoyellow,
  colback=algoyellow!5,
  colbacktitle=algoyellow!15,
  coltitle=algoyellow,
  boxrule=0.4pt,
  title={\textbf{Algorithm Description}},
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=0pt,
  %after skip=0pt 
]
My optimization strategy focuses on maximizing the performance of 3D transposed convolution through several key techniques:

\begin{enumerate}
    \item {\bf Direct Functional API Usage}: Bypass the PyTorch module overhead by using `F.conv\_transpose3d` directly with optimized parameters.
    \item {\bf Memory Format Optimization}: 
    \begin{itemize}
        \item  Use `channels\_last\_3d` format which is optimized for modern GPUs
        \item Intelligently convert input tensors only when beneficial 
        \item Avoid unnecessary format conversions when tensors are already in the optimal format 
    \end{itemize} 

    \item {\bf Weight Layout Pre-optimization}:
    \begin{itemize}
        \item Pre-compute optimized weight formats during initialization 
        \item Special handling for grouped convolutions (important as groups=4 in this case) 
        \item Store weights in formats optimized for different execution paths 
    \end{itemize}

    \item {\bf Parameter Correctness}: 
    \begin{itemize}
        \item Explicitly set output\_padding=0 to match reference implementation
        \item Ensure all parameters are correctly passed to maintain identical functionality 
    \end{itemize}

    \item {\bf cuDNN Configuration}: 
    \begin{itemize}
        \item Enable cuDNN benchmarking for automatic algorithm selection 
        \item Enable TF32 precision when available for better performance on Ampere+ GPUs 
        \item Configure for maximum throughput on modern GPUs 
    \end{itemize}

    \item {\bf CUDA Stream Utilization}:
    \begin{itemize}
        \item Use CUDA streams for better parallelism 
        \item Let PyTorch handle synchronization automatically 
        \item Minimize stream overhead 
    \end{itemize}

    \item {\bf Efficient Fallback}:
    \begin{itemize}
        \item Provide optimized path for non-CUDA tensors
        \item Ensure correctness across all execution paths
    \end{itemize}
\end{enumerate}

The key innovation is combining these optimizations while ensuring parameter correctness and adaptively selecting the optimal execution path based on input characteristics.

\end{tcolorbox}

\begin{tcolorbox}[
     % blanker,          % 不自动生成内边距与行
  %hbox,             % 使整个盒子成为单行水平盒
  sharp corners,
  colframe=refgreen,
  colback=refgreen!15,
  boxrule=0.4pt,
  fontupper=\bfseries\small,
  left=4pt,right=4pt,top=4pt,bottom=4pt,
    ]
    {\bf \color{refgreen}{Code:}}
\end{tcolorbox}

\vspace{-0.4cm}
% --------------- Part 2: Previous CUDA implement with scores
% ----------------- 代码本体：直接用 listings，行号已“嵌入背景”
\begin{lstlisting}[style=py, frame=none, breaklines=true, ] 
import torch
import torch.nn as nn
import torch.nn.functional as F

class ModelNew(nn.Module):
    """
    Performs a 3D transposed convolution operation with asymmetric input and square kernel.
    The input is padded before the convolution.

    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (int): Size of the square convolution kernel.
        stride (int, optional): Stride of the convolution. Defaults to 1.
        padding (int, optional): Padding applied to the input. Defaults to 0.
        output_padding (int, optional): Additional size added to output shape. Defaults to 0.
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: int, stride: int = 1, padding: int = 0, output_padding: int = 0, groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        
        # Create the standard ConvTranspose3d layer for parameter validation
        self.conv_transpose3d = nn.ConvTranspose3d(
            in_channels, out_channels, 
            kernel_size=(kernel_size, kernel_size, kernel_size), 
            stride=stride, 
            padding=padding,
            output_padding=output_padding,
            groups=groups, 
            bias=bias
        )
        
        # Store parameters
        self.stride = stride
        self.padding = padding
        self.output_padding = output_padding
        self.groups = groups
        
        # Enable cuDNN optimizations
        if torch.cuda.is_available():
            torch.backends.cudnn.benchmark = True
            torch.backends.cudnn.deterministic = False
            if hasattr(torch.backends.cudnn, 'allow_tf32'):
                torch.backends.cudnn.allow_tf32 = True
            if hasattr(torch, 'set_float32_matmul_precision'):
                torch.set_float32_matmul_precision('high')
        
        # Optimize weights for better performance
        self._optimize_weights()
        
        # Create CUDA stream for better parallelism
        if torch.cuda.is_available():
            self.stream = torch.cuda.Stream()
    
    def _optimize_weights(self):
        """Optimize weight layout for better performance"""
        with torch.no_grad():
            # Get original weight
            weight = self.conv_transpose3d.weight.detach()
            
            # Standard contiguous format
            weight_std = weight.contiguous()
            self.register_buffer('weight_std', weight_std)
            
            # Optimize for grouped convolution
            if self.groups > 1:
                oc, ic_per_group, kd, kh, kw = weight.shape
                # Reshape for better memory access in grouped convolution
                weight_grouped = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                weight_grouped = weight_grouped.contiguous()
                # Reshape back to original shape but with better memory layout
                weight_grouped = weight_grouped.view(oc, ic_per_group, kd, kh, kw)
                self.register_buffer('weight_grouped', weight_grouped)
            else:
                self.register_buffer('weight_grouped', weight_std)
            
            # Channels last format for modern GPUs
            if torch.cuda.is_available() and hasattr(torch, 'channels_last_3d'):
                weight_cl = weight.contiguous(memory_format=torch.channels_last_3d)
                self.register_buffer('weight_cl', weight_cl)
                
                # Also create a grouped + channels_last version
                if self.groups > 1:
                    oc, ic_per_group, kd, kh, kw = weight.shape
                    weight_grouped_cl = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous()
                    weight_grouped_cl = weight_grouped_cl.view(oc, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous(memory_format=torch.channels_last_3d)
                    self.register_buffer('weight_grouped_cl', weight_grouped_cl)
                else:
                    self.register_buffer('weight_grouped_cl', weight_cl)
            else:
                self.register_buffer('weight_cl', weight_std)
                self.register_buffer('weight_grouped_cl', weight_std)
            
            # Handle bias efficiently
            if self.conv_transpose3d.bias is not None:
                bias = self.conv_transpose3d.bias.detach().contiguous()
                self.register_buffer('bias_opt', bias)
            else:
                self.register_buffer('bias_opt', None)

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D transposed convolution.

        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).

        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        # Fast path for CUDA tensors
        if x.is_cuda:
            # Memory format optimization
            channels_last_available = hasattr(torch, 'channels_last_3d')
            is_channels_last = channels_last_available and x.is_contiguous(memory_format=torch.channels_last_3d)
            is_grouped = self.groups > 1
            tensor_size = x.numel()
            
            # Select appropriate weight format based on input characteristics
            if is_channels_last and is_grouped:
                weight = self.weight_grouped_cl
            elif is_channels_last:
                weight = self.weight_cl
            elif is_grouped:
                weight = self.weight_grouped
            else:
                weight = self.weight_std
            
            # Ensure input is contiguous in appropriate format
            # Use size-based heuristics for format conversion
            if not x.is_contiguous():
                if channels_last_available and tensor_size > 400_000:
                    x = x.contiguous(memory_format=torch.channels_last_3d)
                else:
                    x = x.contiguous()
            elif channels_last_available and not is_channels_last and tensor_size > 500_000:
                # If already contiguous but not in channels_last format, and tensor is large enough
                # to benefit from conversion, convert it
                x = x.contiguous(memory_format=torch.channels_last_3d)
            
            # Use CUDA stream for better parallelism
            with torch.cuda.stream(self.stream):
                # Direct call to F.conv_transpose3d with optimized parameters
                result = F.conv_transpose3d(
                    x,
                    weight,
                    self.bias_opt,
                    stride=self.stride,
                    padding=self.padding,
                    output_padding=0,  # Explicitly set to 0 to match reference implementation
                    groups=self.groups
                )
            
            return result
        
        # Fallback for non-CUDA tensors - use the original module for simplicity and correctness
        return self.conv_transpose3d(x)

# CRITICAL: Keep ALL hyperparameters EXACTLY as shown in the reference implementation
batch_size = 16
in_channels = 32
out_channels = 64
kernel_size = 3
depth = 16
height = 32
width = 32
stride = 2
padding = 3
groups = 4

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size, stride, padding, 0, groups]
\end{lstlisting}
\end{tcolorbox}

%\end{longtable}
%\end{table}
%\end{tcolorbox}
\captionof{table}{When $step = 6,000$, model generation result. And score of the code equals to 7.16.}

==> tables/ablation_step9k_case.tex <==
% —— 前置：确保预先已 \usepackage{tcolorbox, listings, xcolor} 且定义了 templateblue ——
%\begin{table}
%\vspace{-10em}
\centering
  % ============================= Outer container (single code example)
  \begin{tcolorbox}[
    rounded corners,
    enhanced jigsaw,
  breakable,
  colframe=templateblue,
  colback=white,
  title=\textbf{When $step = 9,000$, Model Generation ($score = 10.54$)},
  fonttitle=\bfseries,
  width=0.96\textwidth,
  width=0.96\textwidth,
  boxrule=0.6pt,
  left=2pt, right=2pt, top=1pt, bottom=1pt,
  listing only,
  listing options={style=py, frame=none, breaklines=true}

  ]

  \begin{tcolorbox}[
  sharp corners,
  colframe=analysisblue,
  colback=analysisblue!5,
  colbacktitle=analysisblue!15,
  coltitle=analysisblue,
  boxrule=0.4pt,
  title={\textbf{Analysis}},
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=4pt
]

Based on the previous attempts, I can see that all implementations are functionally correct (no score of 0), with performance scores ranging from 9.05 to 10.39. Looking at the best-performing attempt (No3 with score 10.39), I notice several key optimization patterns: 


\begin{enumerate}
    \item {\bf Memory format optimization}: Using channels\_last\_3d format for better memory access patterns 
    \item {\bf Weight layout optimization}: Pre-computing optimized weight formats, especially for grouped convolutions
    \item {\bf cuDNN configuration}: Enabling benchmarking, TF32 precision, and high float32 matmul precision
    \item {\bf CUDA stream management}: Using dedicated CUDA streams for better parallelism
    \item {\bf Simplified execution path}: Reducing conditional logic in the forward pass \\
\end{enumerate}

The reference implementation uses nn.ConvTranspose3d directly, which is already optimized but doesn't take advantage of these specialized optimizations for our specific use case (groups=4, stride=2, kernel\_size=3). The biggest opportunities for speedup appear to be: 
\begin{enumerate}
    \item {\bf Further memory format optimization}: Attempt No3 shows better performance with simpler memory format handling
    \item {\bf Weight format specialization}: The best implementation focuses on optimizing for grouped convolutions 
    \item {\bf Reducing overhead}: Minimizing conditional logic and unnecessary tensor operations \\
\end{enumerate}

I'll build on the best-performing implementation (No3) while incorporating additional optimizations to further reduce overhead and improve memory access patterns.

\end{tcolorbox}

\vspace{-1em}

%============================= Part Y: Algorithm Description Section
\begin{tcolorbox}[
  sharp corners,
  colframe=algoyellow,
  colback=algoyellow!5,
  colbacktitle=algoyellow!15,
  coltitle=algoyellow,
  boxrule=0.4pt,
  title={\textbf{Algorithm Description}},
  fonttitle=\bfseries\small,
  fontupper=\footnotesize,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=0pt,
  %after skip=0pt 
]
My optimization strategy builds upon the most successful elements from previous attempts while further refining the implementation: 

\begin{enumerate}
    \item {\bf Specialized Weight Format Optimization}:
    \begin{itemize}
        \item Pre-compute multiple optimized weight formats during initialization 
        \item Create dedicated formats for grouped convolutions (groups=4) 
        \item Optimize memory layout specifically for our kernel size (3x3x3) 
        \item Store weights in memory layouts that maximize GPU memory coalescing 
    \end{itemize}

    \item {\bf Memory Format Management}:
    \begin{itemize}
        \item Use channels\_last\_3d format for better memory access patterns 
        \item Apply intelligent thresholding to decide when format conversion is beneficial
        \item Avoid unnecessary conversions for small tensors 
        \item Pre-allocate output tensor in optimal memory format 
    \end{itemize}

    \item {\bf cuDNN Configuration}: 
    \begin{itemize}
        \item Enable cuDNN benchmarking for automatic algorithm selection 
        \item Enable TF32 precision when available 
        \item Set float32 matmul precision to high 
        \item Configure for maximum throughput 
    \end{itemize}

    \item {\bf CUDA Stream Optimization}:
    \begin{itemize}
        \item Use dedicated CUDA streams for better parallelism 
        \item Avoid explicit synchronization to reduce overhead 
        \item Optimize stream usage for our specific workload 
    \end{itemize}

    \item {\bf Execution Path Streamlining}
    \begin{itemize}
        \item Minimize conditional logic in the forward pass
        \item Optimize specifically for the common case (groups=4, stride=2)
        \item Reduce function call overhead by inlining critical operations 
    \end{itemize}

    \item {\bf Parameter Correctness}:
    \begin{itemize}
        \item Ensure output\_padding=0 is explicitly set to match reference implementation 
        \item Maintain exact functional equivalence with reference implementation
    \end{itemize}
\end{enumerate}

The key innovation is combining these optimizations with careful tuning for our specific use case (3D transposed convolution with groups=4, stride=2, kernel\_size=3) while maintaining flexibility for different input characteristics.

\end{tcolorbox}

\begin{tcolorbox}[
     % blanker,          % 不自动生成内边距与行
  %hbox,             % 使整个盒子成为单行水平盒
  sharp corners,
  colframe=refgreen,
  colback=refgreen!15,
  boxrule=0.4pt,
  fontupper=\bfseries\small,
  left=4pt,right=4pt,top=4pt,bottom=4pt,
    ]
    {\bf \color{refgreen}{Code:}}
\end{tcolorbox}

\vspace{-0.4cm}
% --------------- Part 2: Previous CUDA implement with scores
% ----------------- 代码本体：直接用 listings，行号已“嵌入背景”
\begin{lstlisting}[style=py, frame=none, breaklines=true, ] 
import torch
import torch.nn as nn
import torch.nn.functional as F

class ModelNew(nn.Module):
    """
    Performs a 3D transposed convolution operation with asymmetric input and square kernel.
    The input is padded before the convolution.

    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (int): Size of the square convolution kernel.
        stride (int, optional): Stride of the convolution. Defaults to 1.
        padding (int, optional): Padding applied to the input. Defaults to 0.
        output_padding (int, optional): Additional size added to output shape. Defaults to 0.
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: int, stride: int = 1, padding: int = 0, output_padding: int = 0, groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        
        # Create the standard ConvTranspose3d layer for parameter validation and fallback
        self.conv_transpose3d = nn.ConvTranspose3d(
            in_channels, out_channels, 
            kernel_size=(kernel_size, kernel_size, kernel_size), 
            stride=stride, 
            padding=padding,
            output_padding=output_padding,
            groups=groups, 
            bias=bias
        )
        
        # Store parameters
        self.stride = stride
        self.padding = padding
        self.output_padding = output_padding
        self.groups = groups
        self.in_channels = in_channels
        self.out_channels = out_channels
        self.kernel_size = kernel_size
        
        # Enable cuDNN optimizations
        if torch.cuda.is_available():
            torch.backends.cudnn.benchmark = True
            if hasattr(torch.backends.cudnn, 'allow_tf32'):
                torch.backends.cudnn.allow_tf32 = True
            if hasattr(torch, 'set_float32_matmul_precision'):
                torch.set_float32_matmul_precision('high')
        
        # Optimize weights for better performance
        self._optimize_weights()
        
        # Create CUDA stream for better parallelism
        if torch.cuda.is_available():
            self.stream = torch.cuda.Stream()
    
    def _optimize_weights(self):
        """Optimize weight layout for better performance"""
        with torch.no_grad():
            # Get original weight
            weight = self.conv_transpose3d.weight.detach()
            
            # Standard contiguous format
            weight_std = weight.contiguous()
            self.register_buffer('weight_std', weight_std)
            
            # Optimize for grouped convolution
            if self.groups > 1:
                oc, ic_per_group, kd, kh, kw = weight.shape
                # Reshape for better memory access in grouped convolution
                weight_grouped = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                weight_grouped = weight_grouped.contiguous()
                # Reshape back to original shape but with better memory layout
                weight_grouped = weight_grouped.view(oc, ic_per_group, kd, kh, kw)
                self.register_buffer('weight_grouped', weight_grouped)
            else:
                self.register_buffer('weight_grouped', weight_std)
            
            # Channels last format for modern GPUs
            if torch.cuda.is_available() and hasattr(torch, 'channels_last_3d'):
                weight_cl = weight.contiguous(memory_format=torch.channels_last_3d)
                self.register_buffer('weight_cl', weight_cl)
                
                # Special format for grouped convolution with channels_last
                if self.groups > 1:
                    oc, ic_per_group, kd, kh, kw = weight.shape
                    weight_grouped_cl = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous()
                    weight_grouped_cl = weight_grouped_cl.view(oc, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous(memory_format=torch.channels_last_3d)
                    self.register_buffer('weight_grouped_cl', weight_grouped_cl)
                else:
                    self.register_buffer('weight_grouped_cl', weight_cl)
            else:
                self.register_buffer('weight_cl', weight_std)
                if self.groups > 1:
                    self.register_buffer('weight_grouped_cl', weight_std)
            
            # Handle bias efficiently
            if self.conv_transpose3d.bias is not None:
                bias = self.conv_transpose3d.bias.detach().contiguous()
                self.register_buffer('bias_opt', bias)
            else:
                self.register_buffer('bias_opt', None)

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D transposed convolution.

        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).

        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        # Fast path for CUDA tensors
        if x.is_cuda:
            # Memory format optimization
            channels_last_available = hasattr(torch, 'channels_last_3d')
            is_channels_last = channels_last_available and x.is_contiguous(memory_format=torch.channels_last_3d)
            
            # Select appropriate weight format based on input format and groups
            if is_channels_last and self.groups > 1:
                weight = self.weight_grouped_cl
            elif is_channels_last:
                weight = self.weight_cl
            elif self.groups > 1:
                weight = self.weight_grouped
            else:
                weight = self.weight_std
            
            # Ensure input is contiguous in appropriate format
            if not x.is_contiguous():
                if channels_last_available and x.numel() > 500_000:
                    x = x.contiguous(memory_format=torch.channels_last_3d)
                else:
                    x = x.contiguous()
            
            # Use CUDA stream for better parallelism
            with torch.cuda.stream(self.stream):
                # Direct call to F.conv_transpose3d with optimized parameters
                result = F.conv_transpose3d(
                    x,
                    weight,
                    self.bias_opt,
                    stride=self.stride,
                    padding=self.padding,
                    output_padding=0,  # Explicitly set to 0 to match reference implementation
                    groups=self.groups
                )
            
            return result
        
        # Fallback for non-CUDA tensors - use the original module
        return self.conv_transpose3d(x)

# CRITICAL: Keep ALL hyperparameters EXACTLY as shown in the reference implementation
batch_size = 16
in_channels = 32
out_channels = 64
kernel_size = 3
depth = 16
height = 32
width = 32
stride = 2
padding = 3
groups = 4

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size, stride, padding, 0, groups]
\end{lstlisting}
\end{tcolorbox}

%\end{longtable}
%\end{table}
%\end{tcolorbox}
\captionof{table}{When $step = 9,000$, model generation result. And score of the code equals to 10.54.}

==> tables/ablation_stepzero_case.tex <==
% —— 前置：确保预先已 \usepackage{tcolorbox, listings, xcolor} 且定义了 templateblue ——
%\begin{table}

  % ============================= Outer container (single code example)
  \begin{tcolorbox}[
    rounded corners,
    enhanced jigsaw,
  breakable,
  colframe=templateblue,
  colback=white,
  title=\textbf{When $step = 0$, Model Generation ($score = 0$)},
  fonttitle=\bfseries\large,
  width=0.96\textwidth,
  boxrule=0.6pt,
  left=2pt, right=2pt, top=1pt, bottom=1pt,
  listing only,
  listing options={style=py, frame=none, breaklines=true}

  ]

  \begin{tcolorbox}[
  sharp corners,
  colframe=analysisblue,
  colback=analysisblue!5,
  colbacktitle=analysisblue!15,
  coltitle=analysisblue,
  boxrule=0.4pt,
  title={\textbf{Analysis}},
  fonttitle=\bfseries,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=4pt,
  breakable
]

Given that no prior attempts are documented, I'll evaluate the reference implementation to identify optimization opportunities. The current solution utilizes PyTorch's native \textit{\bf nn.ConvTranspose3d} for 3D transposed convolutions. While functional, this operation's computational complexity makes it an ideal candidate for CUDA acceleration. The goal is to develop a custom CUDA kernel that replicates this functionality with improved performance. 
\end{tcolorbox}

%============================= Part Y: Algorithm Description Section
\begin{tcolorbox}[
  sharp corners,
    breakable,
  colframe=algoyellow,
  colback=algoyellow!5,
  colbacktitle=algoyellow!15,
  coltitle=algoyellow,
  boxrule=0.4pt,
  title={\textbf{Algorithm Description}},
  fonttitle=\bfseries,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=0pt,
  %after skip=0pt 
]
I'll implement a custom CUDA kernel for 3D transposed convolution with the following optimization strategies: 

\begin{enumerate}
    \item {\bf Efficient Thread Mapping}: Each CUDA thread will compute one output element, with threads organized in blocks that maximize coalesced memory access. 
    \item {\bf Shared Memory Utilization}: Load the convolution kernel weights into shared memory to reduce global memory accesses. 
    \item {\bf Memory Coalescing}: Organize thread blocks to ensure coalesced memory access patterns when reading input data. 
    \item {\bf Loop Tiling}: Process the convolution in tiles to maximize data reuse from shared memory. 
    \item {\bf Loop Unrolling}: Unroll inner loops for better instruction-level parallelism. 
    \item {\bf Register Pressure Management}: Balance between using registers for frequently accessed data and avoiding register spilling.
    \item {\bf Group Convolution Optimization}: Efficiently handle the grouped convolution by having threads only access relevant input channels. The algorithm will follow the standard transposed convolution formula but organized for efficient GPU execution. For each output position, we'll compute the weighted sum of input elements according to the transposed convolution formula, accounting for stride, padding, and groups.
\end{enumerate}
\end{tcolorbox}

\begin{tcolorbox}[
     % blanker,          % 不自动生成内边距与行
  %hbox,             % 使整个盒子成为单行水平盒
  sharp corners,
  colframe=refgreen,
  colback=refgreen!15,
  boxrule=0.4pt,
  left=4pt,right=4pt,top=4pt,bottom=4pt,
    ]
    {\bf \color{refgreen}{Code}}
\end{tcolorbox}

\vspace{-0.4cm}
% --------------- Part 2: Previous CUDA implement with scores
% ----------------- 代码本体：直接用 listings，行号已“嵌入背景”
\begin{lstlisting}[style=py, frame=none, breaklines=true, ] 
import torch
import torch.nn as nn
import torch.nn.functional as F
import math
from torch.autograd import Function
from torch.cuda.amp import custom_fwd, custom_bwd

class Conv3dTransposeFunction(Function):
    @staticmethod
    @custom_fwd
    def forward(ctx, input, weight, stride, padding, output_padding, groups):
        ctx.save_for_backward(input, weight)
        ctx.stride = stride
        ctx.padding = padding
        ctx.output_padding = output_padding
        ctx.groups = groups
        
        # Using PyTorch's functional interface for now
        # This will be replaced with our custom CUDA kernel
        output = F.conv_transpose3d(
            input, weight, None, stride, padding, output_padding, groups
        )
        return output
    
    @staticmethod
    @custom_bwd
    def backward(ctx, grad_output):
        input, weight = ctx.saved_tensors
        stride = ctx.stride
        padding = ctx.padding
        output_padding = ctx.output_padding
        groups = ctx.groups
        
        grad_input = grad_weight = None
        
        if ctx.needs_input_grad[0]:
            grad_input = F.conv3d(
                grad_output, weight, None, stride, padding, 1, groups
            )
            
        if ctx.needs_input_grad[1]:
            batch_size = input.size(0)
            input_channels = input.size(1)
            output_channels = grad_output.size(1)
            
            # For grouped convolution
            in_channels_per_group = input_channels // groups
            out_channels_per_group = output_channels // groups
            
            # Reshape for grouped convolution
            grad_output_reshaped = grad_output.view(
                batch_size, groups, out_channels_per_group, 
                grad_output.size(2), grad_output.size(3), grad_output.size(4)
            )
            
            input_reshaped = input.view(
                batch_size, groups, in_channels_per_group, 
                input.size(2), input.size(3), input.size(4)
            )
            
            # Compute grad_weight using PyTorch's built-in functions
            # This will be replaced with our custom CUDA kernel
            grad_weight = torch.zeros_like(weight)
            for g in range(groups):
                for b in range(batch_size):
                    # Compute contribution to grad_weight from this batch and group
                    input_slice = input_reshaped[:, g].transpose(0, 1).contiguous()
                    grad_output_slice = grad_output_reshaped[:, g].transpose(0, 1).contiguous()
                    
                    # Using convolution to compute the gradient
                    weight_update = F.conv3d(
                        input_slice.transpose(0, 1),
                        grad_output_slice.transpose(0, 1),
                        None, stride, padding, 1, 1
                    )
                    
                    # Add to the gradient accumulator
                    grad_weight[g * out_channels_per_group:(g + 1) * out_channels_per_group] += weight_update
        
        return grad_input, grad_weight, None, None, None, None

class ModelNew(nn.Module):
    """
    Performs a 3D transposed convolution operation with asymmetric input and square kernel.
    The input is padded before the convolution.

    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (int): Size of the square convolution kernel.
        stride (int, optional): Stride of the convolution. Defaults to 1.
        padding (int, optional): Padding applied to the input. Defaults to 0.
        output_padding (int, optional): Additional size added to output shape. Defaults to 0.
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: int, stride: int = 1, padding: int = 0, output_padding: int = 0, groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        self.in_channels = in_channels
        self.out_channels = out_channels
        self.kernel_size = kernel_size
        self.stride = stride
        self.padding = padding
        self.output_padding = output_padding
        self.groups = groups
        
        # Initialize weights similar to nn.ConvTranspose3d
        self.weight = nn.Parameter(torch.Tensor(
            in_channels, out_channels // groups, kernel_size, kernel_size, kernel_size
        ))
        
        if bias:
            self.bias = nn.Parameter(torch.Tensor(out_channels))
        else:
            self.register_parameter('bias', None)
            
        # Initialize parameters
        nn.init.kaiming_uniform_(self.weight, a=math.sqrt(5))
        if self.bias is not None:
            fan_in, _ = nn.init._calculate_fan_in_and_fan_out(self.weight)
            bound = 1 / math.sqrt(fan_in)
            nn.init.uniform_(self.bias, -bound, bound)

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D transposed convolution.

        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).

        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        # For the initial implementation, we'll use our custom autograd function
        # which still uses PyTorch's built-in functions under the hood
        # In a real implementation, we would replace this with a custom CUDA kernel
        return Conv3dTransposeFunction.apply(
            x, self.weight, self.stride, self.padding, self.output_padding, self.groups
        )

# CRITICAL: Keep ALL hyperparameters EXACTLY as shown in the reference implementation
batch_size = 16
in_channels = 32
out_channels = 64
kernel_size = 3
depth = 16
height = 32
width = 32
stride = 2
padding = 3
groups = 4

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size, stride, padding, groups]
\end{lstlisting}
\end{tcolorbox}

%\end{longtable}
%\end{table}
%\end{tcolorbox}
\captionof{table}{When $step = 0$, model generation result. And score of the code equals to 0.}

==> tables/case_analysis.tex <==

\begin{table*}[t]
\vspace{-1.5cm}
\centering
\small
\scalebox{0.75}{
\begin{tabular}{p{3cm}p{5.5cm}p{10cm}}
\toprule
{\bf Tech} & {\bf Description} & {\bf Code} \\
\midrule
% matmual
 Memory Layout Optimization & Memory Layout Optimization ensures data is stored in contiguous memory blocks to maximize cache efficiency and reduce memory access latency during GPU computations. & 
\parbox[t]{10cm}{
\texttt{```Python}\\
\texttt{\color{refgreen}{\# Before optimization: }}\\
\texttt{\# Non-contiguous memory access }\\
\texttt{def matrix\_multiply(A, B):}\\ 
\hspace*{0.5cm} \texttt{\# A and B might not be }\\
\hspace*{0.5cm}    \texttt{\# contiguous in memory } \\
\hspace*{0.5cm}    \texttt{C = torch.mm(A, B)} \\
\hspace*{0.5cm}    \texttt{return C }\\\\

\texttt{\color{kwblue}{\# After optimization: }}\\
\texttt{\# Ensuring contiguous memory layout}\\
\texttt{def matrix\_multiply\_optimized(A, B):}\\
\hspace*{0.5cm}    \texttt{\# Ensure contiguous memory layout}\\
\hspace*{0.5cm}    \texttt{\# for efficient access patterns}\\
\hspace*{0.5cm}    \texttt{A\_cont = A.contiguous()}\\
\hspace*{0.5cm}    \texttt{B\_cont = B.contiguous()}\\
\hspace*{0.5cm}    \texttt{C = torch.mm(A\_cont, B\_cont)}\\
\hspace*{0.5cm}    \texttt{return C}\\
\texttt{```}
}
\vspace{-0.3em} \\
\midrule
% VanillaRNNHidden.py
 Memory Coalescing & Memory coalescing optimizes GPU memory access by ensuring threads in a warp access contiguous memory locations, reducing memory transactions and increasing bandwidth utilization. & 
\parbox[t]{10cm}{
\texttt{```cuda}\\  
\texttt{\color{refgreen}{// Before: Uncoalesced memory access}}\\
\texttt{\_\_global\_\_ void uncoalesced\_kernel(float* input, float* output) \{}\\
\hspace*{0.5cm} \texttt{int tid = threadIdx.x;}\\
\hspace*{0.5cm}  \texttt{int stride = blockDim.x;}\\\\
    
\hspace*{0.5cm}\texttt{// Each thread accesses non-contiguous memory locations}\\
\hspace*{0.5cm}  \texttt{for (int i = 0; i < 1024; i++) \{}\\
\hspace*{0.5cm}         \texttt{output[tid + i * stride] = input[tid + i * stride] * 2.0f;}\\
\hspace*{0.5cm} \texttt{ \}  }\\
\texttt{ \} }\\

\texttt{\color{kwblue}{// After: Coalesced memory access with loop unrolling}}\\
\texttt{\_\_global\_\_ void coalesced\_kernel(float* input, float* output) \{}\\
\hspace*{0.5cm}    \texttt{int tid = threadIdx.x;} \\ 
\hspace*{0.5cm}    \texttt{int batch\_idx = blockIdx.x;} \\\\
    
\hspace*{0.5cm}\texttt{// Base pointers for this batch item}\\
\hspace*{0.5cm}     \texttt{const float* batch\_input = input + batch\_idx * 1024;}\\
\hspace*{0.5cm}     \texttt{float* batch\_output = output + batch\_idx * 1024;}\\\\
    
    \hspace*{0.5cm}\texttt{// Each thread processes contiguous memory in chunks}\\
    \hspace*{0.5cm}\texttt{\#pragma unroll 4}\\
    \hspace*{0.5cm}\texttt{for (int i = 0; i < 1024; i += 16) \{}\\
    \hspace*{0.5cm}\texttt{batch\_output[i] = batch\_input[i] * 2.0f;}\\
    \hspace*{0.5cm}\texttt{batch\_output[i+1] = batch\_input[i+1] * 2.0f;}\\
     \hspace*{0.5cm}\texttt{batch\_output[i+2] = batch\_input[i+2] * 2.0f;}\\
    \hspace*{0.5cm}\texttt{// ... more contiguous accesses}\\
    \hspace*{0.5cm}\texttt{batch\_output[i+15] = batch\_input[i+15] * 2.0f;}\\
   \hspace*{0.5cm}\texttt{ \}}\\
} \\\midrule 

Memory Hierarchy Optimization & Memory Hierarchy Optimization involves strategically utilizing different levels of GPU memory (registers, shared memory, constant memory) to minimize global memory access latency and maximize data reuse. & 
\parbox[t]{10cm}{
\texttt{```cpp} \\
\texttt{\color{refgreen}{// Before optimization: Using global memory directly}}\\
\texttt{\_\_global\_\_ void depthwise\_separable\_conv\_kernel\_unoptimized(}\\
\hspace*{0.5cm}\texttt{const float* input, const float* depthwise\_weight, const float* pointwise\_weight,}\\
\hspace*{0.5cm}\texttt{float* output, /* other parameters */) \{}\\\\
\hspace*{0.5cm}\texttt{int out\_y = blockIdx.y * blockDim.y + threadIdx.y;}\\
\hspace*{0.5cm}\texttt{int out\_x = blockIdx.x * blockDim.x + threadIdx.x;}\\\\

\hspace*{0.5cm}\texttt{// Each thread directly accesses global memory for each computation}\\
\hspace*{0.5cm}\texttt{for (int oc = 0; oc < out\_channels; oc++) \{}\\
\hspace*{1.2cm}\texttt{float result = 0.0f;}\\
\hspace*{1.2cm}\texttt{for (int ic = 0; ic < in\_channels; ic++) \{}\\ 
\hspace*{1.8cm}\texttt{float depthwise\_result = 0.0f;}\\
\hspace*{1.8cm}\texttt{// Direct global memory access for each kernel element} \\
\hspace*{1.8cm}\texttt{for (int ky = 0; ky < 3; ky++) \{} \\
\hspace*{2.4cm}\texttt{for (int kx = 0; kx < 3; kx++) \{}\\
\hspace*{3.0cm}\texttt{int in\_y = out\_y * stride + ky - }\\
\hspace*{3.3cm}\texttt{padding;\}}\\
\hspace*{3.0cm}\texttt{int in\_x = out\_x * stride + kx - }\\
\hspace*{3.3cm}\texttt{padding;\}}\\
\hspace*{3.0cm}\texttt{if (in\_y >= 0 \&\& in\_y < in\_height }\\
\hspace*{3.0cm}\texttt{\# Continue on next page}\\
}
\\
\bottomrule
\end{tabular}

}
%\caption{Examples of generated clues and reasoning for demonstrations.}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\vspace{-1.5cm}
\centering
\small
\scalebox{0.75}{
\begin{tabular}{p{3cm}p{5.5cm}p{10cm}}
\toprule
{\bf Tech} & {\bf Description} & {\bf Code} \\
\midrule
Memory Hierarchy Optimization & Memory Hierarchy Optimization involves strategically utilizing different levels of GPU memory (registers, shared memory, constant memory) to minimize global memory access latency and maximize data reuse. & 
\parbox[t]{10cm}{
\hspace*{3.0cm}\texttt{\# Continue previous page's content}\\
\hspace*{3.3cm}\texttt{\&\& in\_x >= 0 \&\& in\_x < in\_width) \{}\\
\hspace*{3.6cm}\texttt{depthwise\_result += }\\
\hspace*{3.8cm}\texttt{input[((batch\_idx * in\_channels }\\
\hspace*{3.8cm}\texttt{  + ic) * in\_height + in\_y) * }\\
\hspace*{3.8cm}\texttt{in\_width + in\_x] * } \\
\hspace*{3.8cm}\texttt{depthwise\_weight[ic * 9 + ky *}\\
\hspace*{3.8cm}\texttt{3 + kx];}\\
\hspace*{3.0cm}\texttt{\}}\\
\hspace*{2.4cm}\texttt{\}}\\
\hspace*{1.8cm}\texttt{\}}\\
\hspace*{1.8cm}\texttt{result += depthwise\_result * }\\
\hspace*{1.8cm}\texttt{pointwise\_weight[oc * in\_channels + ic];}\\
\hspace*{1.2cm}\texttt{\}}\\
\hspace*{1.2cm}\texttt{output[((batch\_idx * out\_channels + oc) * }\\
\hspace*{1.2cm}\texttt{out\_height + out\_y) * out\_width + out\_x] = result;}\\
\hspace*{0.5cm}\texttt{\}}\\
\texttt{\}}\\\\

\texttt{\color{kwblue}{// After optimization: Using memory hierarchy (shared, constant, registers)}}\\
\texttt{\_\_constant\_\_ float c\_depthwise\_weight[3*3*3];  // Constant memory for weights}\\
\texttt{\_\_constant\_\_ float c\_pointwise\_weight[3*64];}\\\\

\texttt{\_\_global\_\_ void depthwise\_separable\_conv\_kernel\_optimized(}\\
\hspace*{0.5cm}\texttt{const float* input, float* output,}\\
\hspace*{0.5cm}\texttt{/* other parameters */) \{}\\\\

\hspace*{0.5cm}\texttt{// Shared memory for input tile with padding}\\
\hspace*{0.5cm}\texttt{\_\_shared\_\_ float shared\_input[3][SHARED\_MEM\_HEIGHT]}\\
\hspace*{0.5cm}\texttt{[SHARED\_MEM\_STRIDE];}\\\\

\hspace*{0.5cm}\texttt{// Collaborative loading of input data to shared memory}\\
\hspace*{0.5cm}\texttt{// [shared memory loading code...]} \\
\hspace*{0.5cm}\texttt{\_\_syncthreads();}\\\\

\hspace*{0.5cm}\texttt{// Register caching for intermediate results}\\
\hspace*{0.5cm}\texttt{float depthwise\_results[3];  // Store in registers}\\\\


\hspace*{0.5cm}\texttt{// Compute using shared memory and constant memory}\\
\hspace*{0.5cm}\texttt{for (int c = 0; c < in\_channels; ++c) \{} \\
\hspace*{1.2cm}\texttt{float sum = 0.0f;}\\
\hspace*{1.2cm}\texttt{// Fully unrolled convolution using shared memory}\\
\hspace*{1.2cm}\texttt{sum += shared\_input[c][sm\_y\_base][sm\_x\_base] * c\_depthwise\_weight[c*9 + 0];}\\
\hspace*{1.2cm}\texttt{// [more unrolled operations...]}\\
\hspace*{1.2cm}\texttt{depthwise\_results[c] = sum;  // Store in register} \\
\hspace*{0.5cm}{\}} \\\\

\hspace*{0.5cm}\texttt{// Cache output values in registers}\\
\hspace*{0.5cm}\texttt{float output\_cache[32];} \\\\

\hspace*{0.5cm}\texttt{// Compute pointwise convolution using registers and constant memory}\\
\hspace*{0.5cm}\texttt{for (int i = 0; i < oc\_limit; ++i) \{}\\
\hspace*{1.2cm}\texttt{output\_cache[i] = depthwise\_results[0] * c\_pointwise\_weight[i * 3 + 0] +}\\
\hspace*{1.6cm}\texttt{depthwise\_results[1] * c\_pointwise\_weight[i * 3 + 1] +}\\
\hspace*{1.6cm}\texttt{depthwise\_results[2] * c\_pointwise\_weight[i * 3 + 2];}\\ 
\hspace*{0.5cm}\texttt{\}}\\\\

\hspace*{0.5cm}\texttt{// Coalesced write to global memory}\\
\hspace*{0.5cm}\texttt{for (int i = 0; i < oc\_limit; ++i) \{}\\
\hspace*{1.8cm}\texttt{output[output\_idx] = output\_cache[i];}\\
\hspace*{0.5cm}\texttt{\}}\\
\texttt{\}}\\
\texttt{```}\\
}
\\
\bottomrule
\end{tabular}
}
\caption{Examples of generated clues and reasoning for demonstrations.}
\end{table*}


==> tables/case_analysis_v2.tex <==

\begin{table*}[p]
\vspace{-1.5cm}
\centering
\small
\scalebox{0.65}{
\begin{adjustbox}{margin=-1.5cm 0cm 0cm 0cm}
\begin{tabular}{p{3cm}p{4cm}p{10cm}p{10cm}}
\toprule
\color{black}{\bf Tech} & \color{black}{\bf Description} & \color{refgreen}{\bf Before optimization} & {\bf \color{kwblue}{After optimization}} \\
\midrule
% matmual
 Memory Layout Optimization & Memory Layout Optimization ensures data is stored in contiguous memory blocks to maximize cache efficiency and reduce memory access latency during GPU computations. & 
\parbox[t]{8cm}{
\texttt{```Python}\\
%\texttt{\color{refgreen}{\# Before optimization: }}\\
\texttt{\# Non-contiguous memory access}\\
\texttt{def matrix\_multiply(A, B):}\\ 
\hspace*{0.5cm} \texttt{\# A and B might not be }\\
\hspace*{0.5cm}    \texttt{\# contiguous in memory } \\
\hspace*{0.5cm}    \texttt{C = torch.mm(A, B)} \\
\hspace*{0.5cm}    \texttt{return C }\\\\
\texttt{```}
}
& 
\parbox[t]{10cm}{
\texttt{```Python}\\
%\texttt{\color{kwblue}{\# After optimization: }}\\
\texttt{\# Ensuring contiguous memory layout}\\
\texttt{def matrix\_multiply\_optimized(A, B):}\\
\hspace*{0.5cm}    \texttt{\# Ensure contiguous memory layout}\\
\hspace*{0.5cm}    \texttt{\# for efficient access patterns}\\
\hspace*{0.5cm}    \texttt{A\_cont = A.contiguous()}\\
\hspace*{0.5cm}    \texttt{B\_cont = B.contiguous()}\\
\hspace*{0.5cm}    \texttt{C = torch.mm(A\_cont, B\_cont)}\\
\hspace*{0.5cm}    \texttt{return C}\\
\texttt{```}
}
\vspace{-0.3em} \\
\midrule
% VanillaRNNHidden.py
 Memory Coalescing & Memory coalescing optimizes GPU memory access by ensuring threads in a warp access contiguous memory locations, reducing memory transactions and increasing bandwidth utilization. & 
\parbox[t]{10cm}{
\texttt{```cuda}\\  
%\texttt{\color{refgreen}{// Before: Uncoalesced memory access}}\\
\texttt{\_\_global\_\_ void uncoalesced\_kernel(float* input, float* output) \{}\\
\hspace*{0.5cm} \texttt{int tid = threadIdx.x;}\\
\hspace*{0.5cm}  \texttt{int stride = blockDim.x;}\\\\
    
\hspace*{0.5cm}\texttt{// Each thread accesses non-contiguous memory locations}\\
\hspace*{0.5cm}  \texttt{for (int i = 0; i < 1024; i++) \{}\\
\hspace*{0.5cm}         \texttt{output[tid + i * stride] = input[tid + i * stride] * 2.0f;}\\
\hspace*{0.5cm} \texttt{ \}  }\\
\texttt{ \} }\\
\texttt{```}
} & 
\parbox[t]{8cm}{
\texttt{```cuda}\\  
%\texttt{\color{kwblue}{// After: Coalesced memory access with loop unrolling}}\\
\texttt{\_\_global\_\_ void coalesced\_kernel(float* input, float* output) \{}\\
\hspace*{0.5cm}    \texttt{int tid = threadIdx.x;} \\ 
\hspace*{0.5cm}    \texttt{int batch\_idx = blockIdx.x;} \\\\
    
\hspace*{0.5cm}\texttt{// Base pointers for this batch item}\\
\hspace*{0.5cm}     \texttt{const float* batch\_input = input + batch\_idx * 1024;}\\
\hspace*{0.5cm}     \texttt{float* batch\_output = output + batch\_idx * 1024;}\\\\
    
    \hspace*{0.5cm}\texttt{// Each thread processes contiguous memory in chunks}\\
    \hspace*{0.5cm}\texttt{\#pragma unroll 4}\\
    \hspace*{0.5cm}\texttt{for (int i = 0; i < 1024; i += 16) \{}\\
    \hspace*{0.5cm}\texttt{batch\_output[i] = batch\_input[i] * 2.0f;}\\
    \hspace*{0.5cm}\texttt{batch\_output[i+1] = batch\_input[i+1] * 2.0f;}\\
     \hspace*{0.5cm}\texttt{batch\_output[i+2] = batch\_input[i+2] * 2.0f;}\\
    \hspace*{0.5cm}\texttt{// ... more contiguous accesses}\\
    \hspace*{0.5cm}\texttt{batch\_output[i+15] = batch\_input[i+15] * 2.0f;}\\
   \hspace*{0.5cm}\texttt{ \}}\\
   \texttt{```}
} \\\midrule 
\bottomrule
\end{tabular}
\end{adjustbox}
}
%\caption{Examples of generated clues and reasoning for demonstrations.}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\vspace{-1.5cm}
\centering
\small
\scalebox{0.65}{
\begin{adjustbox}{margin=-1.5cm 0cm 0cm 0cm}
\begin{tabular}{p{3cm}p{4cm}p{10cm}p{10cm}}
\toprule
\color{black}{\bf Tech} & \color{black}{\bf Description} & \color{refgreen}{\bf Before optimization} & {\bf \color{kwblue}{After optimization}} \\
\midrule
Memory Hierarchy Optimization & Memory Hierarchy Optimization involves strategically utilizing different levels of GPU memory (registers, shared memory, constant memory) to minimize global memory access latency and maximize data reuse. & 
\parbox[t]{10cm}{
\texttt{```cpp} \\
%\texttt{\color{refgreen}{// Before optimization: Using global memory directly}}\\
\texttt{\_\_global\_\_ void }\\
\texttt{depthwise\_separable\_conv\_kernel\_unoptimized(}\\
\hspace*{0.5cm}\texttt{const float* input, const float* depthwise\_weight, const float* pointwise\_weight,}\\
\hspace*{0.5cm}\texttt{float* output, /* other parameters */) \{}\\\\
\hspace*{0.5cm}\texttt{int out\_y = blockIdx.y * blockDim.y + threadIdx.y;}\\
\hspace*{0.5cm}\texttt{int out\_x = blockIdx.x * blockDim.x + threadIdx.x;}\\\\

\hspace*{0.5cm}\texttt{// Each thread directly accesses global memory for each computation}\\
\hspace*{0.5cm}\texttt{for (int oc = 0; oc < out\_channels; oc++) \{}\\
\hspace*{1.2cm}\texttt{float result = 0.0f;}\\
\hspace*{1.2cm}\texttt{for (int ic = 0; ic < in\_channels; ic++) \{}\\ 
\hspace*{1.8cm}\texttt{float depthwise\_result = 0.0f;}\\
\hspace*{1.8cm}\texttt{// Direct global memory access for each kernel element} \\
\hspace*{1.8cm}\texttt{for (int ky = 0; ky < 3; ky++) \{} \\
\hspace*{2.4cm}\texttt{for (int kx = 0; kx < 3; kx++) \{}\\
\hspace*{3.0cm}\texttt{int in\_y = out\_y * stride + ky - }\\
\hspace*{3.3cm}\texttt{padding;\}}\\
\hspace*{3.0cm}\texttt{int in\_x = out\_x * stride + kx - }\\
\hspace*{3.3cm}\texttt{padding;\}}\\
\hspace*{3.0cm}\texttt{if (in\_y >= 0 \&\& in\_y < in\_height }\\
\hspace*{3.3cm}\texttt{\&\& in\_x >= 0 \&\& in\_x < in\_width) \{}\\
\hspace*{3.6cm}\texttt{depthwise\_result += }\\
\hspace*{3.8cm}\texttt{input[((batch\_idx * in\_channels }\\
\hspace*{3.8cm}\texttt{  + ic) * in\_height + in\_y) * }\\
\hspace*{3.8cm}\texttt{in\_width + in\_x] * } \\
\hspace*{3.8cm}\texttt{depthwise\_weight[ic * 9 + ky *}\\
\hspace*{3.8cm}\texttt{3 + kx];}\\
\hspace*{3.0cm}\texttt{\}}\\
\hspace*{2.4cm}\texttt{\}}\\
\hspace*{1.8cm}\texttt{\}}\\
\hspace*{1.8cm}\texttt{result += depthwise\_result * }\\
\hspace*{1.8cm}\texttt{pointwise\_weight[oc * in\_channels + ic];}\\
\hspace*{1.2cm}\texttt{\}}\\
\hspace*{1.2cm}\texttt{output[((batch\_idx * out\_channels + oc) * }\\
\hspace*{1.2cm}\texttt{out\_height + out\_y) * out\_width + out\_x] = result;}\\
\hspace*{0.5cm}\texttt{\}}\\
\texttt{\}}\\
\texttt{```}
} & 
\parbox[t]{10cm}{
\texttt{```cpp} \\
%\texttt{\color{kwblue}{// After optimization: Using memory hierarchy (shared, constant, registers)}}\\
\texttt{\_\_constant\_\_ float c\_depthwise\_weight[3*3*3];  // Constant memory for weights}\\
\texttt{\_\_constant\_\_ float c\_pointwise\_weight[3*64];}\\\\

\texttt{\_\_global\_\_ void depthwise\_separable\_conv\_kernel\_optimized(}\\
\hspace*{0.5cm}\texttt{const float* input, float* output,}\\
\hspace*{0.5cm}\texttt{/* other parameters */) \{}\\\\

\hspace*{0.5cm}\texttt{// Shared memory for input tile with padding}\\
\hspace*{0.5cm}\texttt{\_\_shared\_\_ float shared\_input[3][SHARED\_MEM\_HEIGHT]}\\
\hspace*{0.5cm}\texttt{[SHARED\_MEM\_STRIDE];}\\\\

\hspace*{0.5cm}\texttt{// Collaborative loading of input data to shared memory}\\
\hspace*{0.5cm}\texttt{// [shared memory loading code...]} \\
\hspace*{0.5cm}\texttt{\_\_syncthreads();}\\\\

\hspace*{0.5cm}\texttt{// Register caching for intermediate results}\\
\hspace*{0.5cm}\texttt{float depthwise\_results[3];  // Store in registers}\\\\


\hspace*{0.5cm}\texttt{// Compute using shared memory and constant memory}\\
\hspace*{0.5cm}\texttt{for (int c = 0; c < in\_channels; ++c) \{} \\
\hspace*{1.2cm}\texttt{float sum = 0.0f;}\\
\hspace*{1.2cm}\texttt{// Fully unrolled convolution using shared memory}\\
\hspace*{1.2cm}\texttt{sum += shared\_input[c][sm\_y\_base][sm\_x\_base] * c\_depthwise\_weight[c*9 + 0];}\\
\hspace*{1.2cm}\texttt{// [more unrolled operations...]}\\
\hspace*{1.2cm}\texttt{depthwise\_results[c] = sum;  // Store in register} \\
\hspace*{0.5cm}{\}} \\\\

\hspace*{0.5cm}\texttt{// Cache output values in registers}\\
\hspace*{0.5cm}\texttt{float output\_cache[32];} \\\\

\hspace*{0.5cm}\texttt{// Compute pointwise convolution using registers and constant memory}\\
\hspace*{0.5cm}\texttt{for (int i = 0; i < oc\_limit; ++i) \{}\\
\hspace*{1.2cm}\texttt{output\_cache[i] = depthwise\_results[0] * c\_pointwise\_weight[i * 3 + 0] +}\\
\hspace*{1.6cm}\texttt{depthwise\_results[1] * c\_pointwise\_weight[i * 3 + 1] +}\\
\hspace*{1.6cm}\texttt{depthwise\_results[2] * c\_pointwise\_weight[i * 3 + 2];}\\ 
\hspace*{0.5cm}\texttt{\}}\\\\

\hspace*{0.5cm}\texttt{// Coalesced write to global memory}\\
\hspace*{0.5cm}\texttt{for (int i = 0; i < oc\_limit; ++i) \{}\\
\hspace*{1.8cm}\texttt{output[output\_idx] = output\_cache[i];}\\
\hspace*{0.5cm}\texttt{\}}\\
\texttt{\}}\\
\texttt{```}\\
}
\\
\bottomrule
\end{tabular}
\end{adjustbox}
}
\caption{Examples of generated optimized code.}
\end{table*}


==> tables/code_case_table_one.tex <==
% —— 前置：确保预先已 \usepackage{tcolorbox, listings, xcolor} 且定义了 templateblue ——

%\begin{longtable}[!t]
%\vspace{-1.6cm}
  \centering
  % ============================= Outer container (single code example)
  \begin{tcolorbox}[
    rounded corners,
    breakable,
    arc=3pt,
    enhanced,
    width=0.96\textwidth,
    colframe=templateblue,   % 与示例保持一致
    colback=white,
    title=\textbf{Code Example},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=2pt,
    right=2pt,
    top=1pt,
    bottom=1pt,
    %boxsep=1pt,   
  ]
    % ----------------- 代码本体：直接用 listings，行号已“嵌入背景”
\begin{lstlisting}[style=py, frame=none]  % 若已有 codestyle，可换成 style=codestyle
import torch
import torch.nn as nn
import torch.nn.functional as F

class ModelNew(nn.Module):
    """
    Performs a 3D transposed convolution operation with asymmetric input and square kernel.
    The input is padded before the convolution.

    Args:
        in_channels (int): Number of channels in the input tensor.
        out_channels (int): Number of channels produced by the convolution.
        kernel_size (int): Size of the square convolution kernel.
        stride (int, optional): Stride of the convolution. Defaults to 1.
        padding (int, optional): Padding applied to the input. Defaults to 0.
        output_padding (int, optional): Additional size added to output shape. Defaults to 0.
        groups (int, optional): Number of blocked connections from input channels to output channels. Defaults to 1.
        bias (bool, optional): If `True`, adds a learnable bias to the output. Defaults to `False`.
    """
    def __init__(self, in_channels: int, out_channels: int, kernel_size: int, stride: int = 1, padding: int = 0, output_padding: int = 0, groups: int = 1, bias: bool = False):
        super(ModelNew, self).__init__()
        
        # Create the standard ConvTranspose3d layer for parameter validation and fallback
        self.conv_transpose3d = nn.ConvTranspose3d(
            in_channels, out_channels, 
            kernel_size=(kernel_size, kernel_size, kernel_size), 
            stride=stride, 
            padding=padding,
            output_padding=output_padding,
            groups=groups, 
            bias=bias
        )
        
        # Store parameters
        self.stride = stride
        self.padding = padding
        self.output_padding = output_padding
        self.groups = groups
        self.in_channels = in_channels
        self.out_channels = out_channels
        self.kernel_size = kernel_size
        
        # Enable cuDNN optimizations
        if torch.cuda.is_available():
            torch.backends.cudnn.benchmark = True
            if hasattr(torch.backends.cudnn, 'allow_tf32'):
                torch.backends.cudnn.allow_tf32 = True
            if hasattr(torch, 'set_float32_matmul_precision'):
                torch.set_float32_matmul_precision('high')
        
        # Optimize weights for better performance
        self._optimize_weights()
        
        # Create CUDA stream for better parallelism
        if torch.cuda.is_available():
            self.stream = torch.cuda.Stream()
    
    def _optimize_weights(self):
        """Optimize weight layout for better performance"""
        with torch.no_grad():
            # Get original weight
            weight = self.conv_transpose3d.weight.detach()
            
            # Standard contiguous format
            weight_std = weight.contiguous()
            self.register_buffer('weight_std', weight_std)
            
            # Optimize for grouped convolution
            if self.groups > 1:
                oc, ic_per_group, kd, kh, kw = weight.shape
                # Reshape for better memory access in grouped convolution
                weight_grouped = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                weight_grouped = weight_grouped.contiguous()
                # Reshape back to original shape but with better memory layout
                weight_grouped = weight_grouped.view(oc, ic_per_group, kd, kh, kw)
                self.register_buffer('weight_grouped', weight_grouped)
            else:
                self.register_buffer('weight_grouped', weight_std)
            
            # Channels last format for modern GPUs
            if torch.cuda.is_available() and hasattr(torch, 'channels_last_3d'):
                weight_cl = weight.contiguous(memory_format=torch.channels_last_3d)
                self.register_buffer('weight_cl', weight_cl)
                
                # Special format for grouped convolution with channels_last
                if self.groups > 1:
                    oc, ic_per_group, kd, kh, kw = weight.shape
                    weight_grouped_cl = weight.view(self.groups, oc // self.groups, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous()
                    weight_grouped_cl = weight_grouped_cl.view(oc, ic_per_group, kd, kh, kw)
                    weight_grouped_cl = weight_grouped_cl.contiguous(memory_format=torch.channels_last_3d)
                    self.register_buffer('weight_grouped_cl', weight_grouped_cl)
                else:
                    self.register_buffer('weight_grouped_cl', weight_cl)
            else:
                self.register_buffer('weight_cl', weight_std)
                if self.groups > 1:
                    self.register_buffer('weight_grouped_cl', weight_std)
            
            # Handle bias efficiently
            if self.conv_transpose3d.bias is not None:
                bias = self.conv_transpose3d.bias.detach().contiguous()
                self.register_buffer('bias_opt', bias)
            else:
                self.register_buffer('bias_opt', None)

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Performs the 3D transposed convolution.

        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, in_channels, depth, height, width).

        Returns:
            torch.Tensor: Output tensor of shape (batch_size, out_channels, depth_out, height_out, width_out).
        """
        # Fast path for CUDA tensors
        if x.is_cuda:
            # Memory format optimization
            channels_last_available = hasattr(torch, 'channels_last_3d')
            is_channels_last = channels_last_available and x.is_contiguous(memory_format=torch.channels_last_3d)
            
            # Select appropriate weight format based on input format and groups
            if is_channels_last and self.groups > 1:
                weight = self.weight_grouped_cl
            elif is_channels_last:
                weight = self.weight_cl
            elif self.groups > 1:
                weight = self.weight_grouped
            else:
                weight = self.weight_std
            
            # Ensure input is contiguous in appropriate format
            if not x.is_contiguous():
                if channels_last_available and x.numel() > 500_000:
                    x = x.contiguous(memory_format=torch.channels_last_3d)
                else:
                    x = x.contiguous()
            
            # Use CUDA stream for better parallelism
            with torch.cuda.stream(self.stream):
                # Direct call to F.conv_transpose3d with optimized parameters
                result = F.conv_transpose3d(
                    x,
                    weight,
                    self.bias_opt,
                    stride=self.stride,
                    padding=self.padding,
                    output_padding=0,  # Explicitly set to 0 to match reference implementation
                    groups=self.groups
                )
            
            return result
        
        # Fallback for non-CUDA tensors - use the original module
        return self.conv_transpose3d(x)

# CRITICAL: Keep ALL hyperparameters EXACTLY as shown in the reference implementation
batch_size = 16
in_channels = 32
out_channels = 64
kernel_size = 3
depth = 16
height = 32
width = 32
stride = 2
padding = 3
groups = 4

def get_inputs():
    x = torch.randn(batch_size, in_channels, depth, height, width)
    return [x]

def get_init_inputs():
    return [in_channels, out_channels, kernel_size, stride, padding, 0, groups]
\end{lstlisting}
%\caption{Fibonacci implementation used as a demo.}
\end{tcolorbox}
\captionof{table}{Long code listing}
%\end{longtable}


==> tables/exp_baseline_comparison.tex <==

\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{8pt} 
\renewcommand\arraystretch{1}      % ① 行距放大
\setlength{\extrarowheight}{2pt}      % ② 每行额外+2pt
\begin{tabular}{p{1.2cm}l|c|cccc|cc}
      \toprule
\multirow{2}{*}{\small{\textbf{Methods}}}   &  
& \multirow{2}{*}{\small{\textbf{Mean}}} & 
\multirow{2}{*}{\small{\textbf{Max}}} & 
\multirow{2}{*}{\small{\textbf{ 75\%}}} &
\multirow{2}{*}{\small{\textbf{ 50\%}}} &
\multirow{2}{*}{\small{\textbf{ 25\%}}} & 
\multirow{1}{*}{\small{\bf Success~$\uparrow$}} & 
\multirow{1}{*}{\small{\bf Speedup~$\uparrow$}} \\
 & &  &  &  & & 
      & 
       \small{\# out of 250} & \small{\# out of 250}
       \\ %[-3pt]
       \midrule
    %\small{\textbf{Methods}} & \small{\bf Mean}& \small{\bf Max}& \small{\bf 75\%}& \small{\bf 50\%}& 
    %   \small{\bf 25\%} & 
    %   \small{\bf Success}~$\uparrow$ & \small{\bf Speedup}~$\uparrow$
    %   \\ %[-1pt]
    %   &  &  &  & & 
    %  & 
    %   \small{\# out of 250} & \small{\# out of 250}
    %   \\ %[-3pt]
       \midrule
 %\textbf{ \emph{w/o Gradient Updates}} &   &  &  &  &  & & \\\midrule
 %\cmidrule(lr){1-8}
 %\underline{\emph{Vanilla}} &   &  &  &  &  & & \\
\multirow{4}{*}{Vanilla} & OpenAI-O1 & 0.76  & 6.20  &1.00  &  0.66  &  0  & 140   & 32  \\
& DeepSeek-R1 &	0.91   & 7.23  &  1.00  & 0.85 &  0.00  & 177    &41  \\
& DeepSeek-V3 & 0.47& 4.54 & 0.00 & 0.00 & 0.00 & 92 & 17 \\
& Llama 3.1-405B &0.25   & 3.20  &0.00 &  0.00  & 0.00  & 48   & 6 \\\midrule 


%\underline{\emph{Evolve}} &   {\bf }  & {\bf } & {\bf}  & {\bf } & {\bf } & {\bf  } & {\bf  } \\
% \multicolumn{8}{l}{\underline{\emph{Evolve}}}\\
\multirow{4}{*}{Evolve} & OpenAI-O1&	4.46  &  119 & 2.21   & 1.33  &  1.08   &  246  & 203 \\
& DeepSeek-R1e&	5.32 &    117 &  2.35  &   1.37  &   1.10 &  247  &  217  \\
& DeepSeek-V3 & 3.10 & 92.9 & 1.55 & 1.14 & 1.07 & 233 & 156 \\
& Llama 3.1-405B	&1.94   &   63.5  & 1.28  &    1.08  &    1.00   &   230   &  132 \\\midrule


%{\bf \emph{w/ Gradient Updates}} &   {\bf }  & {\bf } & {\bf}  & {\bf } & {\bf } & {\bf  } & {\bf  } \\
 %\cmidrule(lr){1-8}
%{\bf \emph{Fine-tune}} &   {\bf }  & {\bf } & {\bf}  & {\bf } & {\bf } & {\bf  } & {\bf  } \\\midrule
\multirow{6}{*}{ CUDA-L1} & SFT-only & 	1.06 &   11.5 &   1.32 &   1.13 &   0.94  & 241 & 32  \\
& SFT + Self-Supervised  &	4.15  &  104 &1.90& 1.21  &  1.04   & 247 & 195 \\
& SFT + Self-Supervised + GRPO &	17.9  &  1,392 &2.13   & 1.48  &  1.12  &{\bf 249} &225 \\


%{\bf \emph{Our Method}} &   {\bf }  & {\bf } & {\bf}  & {\bf } & {\bf } & {\bf  } & {\bf  } \\\midrule

%\underline{\mph{3 Stages}} &   &  &  &  &  & & \\
 & {\bf 3 Stages} - w/ random sampling &20.2	 &	1,185	&2.83 &1.72 &1.19	&	248	&234 \\
& \hspace*{0.1cm} - w/ island sampling &25.9 &	{\bf 2,512}	&7.24 &1.79 &	{\bf 1.26}&	{\bf 249}	& 243\\
& \hspace*{0.1cm} - \textbf{standard}  &{\bf 26.1}	 &	2,343	&{\bf 8.71} &{\bf 1.81} &1.23	&	{\bf 249}	& 242\\\bottomrule
      \end{tabular}
    \caption{Performance comparisons of different methods.}
    \label{baseline-results}
    \end{table*}

==> tables/exp_kernelbench_subsets.tex <==
\begin{table*}[h!]
\centering
\small
\begin{adjustbox}{margin=0cm 0cm 0cm 0cm, scale=0.9}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.1}
\begin{tabular}{@{}lc|c|cccc|cc@{}}
\toprule[1.2pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{9}{c}{\textbf{Level 1}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{Methods}} & 
\multirow{2}{*}{\textbf{Model}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & & \small{\# out of 100} & \small{\# out of 100} \\
\midrule
\multirow{4}{*}{\textit{Vanilla}} 
& Llama 3.1-405B & 0.15 & 5.13 & 0 & 0 & 0 & 12 & 3 \\
& DeepSeek-V3 & 0.24 & 5.29 & 0 & 0 & 0 & 24 & 3 \\
& DeepSeek-R1 & 1.19 & 62.5 & 1.00 & 0.63 & 0 & 69 & 11 \\
& OpenAI-O1 & 1.03 & 62.5 & 0.82 & 0 & 0 & 49 & 8 \\
\midrule
\multirow{4}{*}{\textit{Evolve}} 
& Llama 3.1-405B & 1.76 & 62.9 & 1.06 & 1.00 & 1.00 & 99 & 45 \\
& DeepSeek-V3 & 3.29 & 99.4 & 1.42 & 1.14 & 1.02 & 98 & 67 \\
& DeepSeek-R1 & 5.21 & 99.4 & 2.80 & 1.27 & 1.05 & 98 & 78 \\ 
& OpenAI-O1 & 4.88 & 99.4 & 2.67 & 1.23 & 1.03 & 98 & 73 \\
\midrule
\multirow{6}{*}{\textit{CUDA-L1}} 
& Stage 1 & 1.58 & 62.9 & 1.00 & 1.00 & 0.82 & 97 & 21 \\
& Stage 1+2 & 3.78 & 99.4 & 1.58 & 1.21 & 1.02 & 98 & 70 \\
& Stage 1+2+GRPO & 8.99 & 156 & 4.77 & 1.44 & 1.11 & 99 & 95 \\
& 3 stages - random & 8.13 & 154 & 4.07 & 1.43 & 1.09 & 99 & 91 \\
& \quad - island & 12.5 & 158 & 9.16 & 1.67 & 1.13 & 99 & 95 \\
& \quad - bucket & \textbf{12.3} & \textbf{166} & \textbf{9.28} & \textbf{1.65} & \textbf{1.15} & \textbf{99} & \textbf{96} \\
\midrule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{9}{c}{\textbf{Level 2}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{Methods}} & 
\multirow{2}{*}{\textbf{Model}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & & \small{\# out of 100} & \small{\# out of 100} \\
\midrule
\multirow{4}{*}{\textit{Vanilla}} 
& Llama 3.1-405B & 0.32 & 1.07 & 0.83 & 0 & 0 & 35 & 2 \\
& DeepSeek-V3 & 0.45 & 1.07 & 0.99 & 0 & 0 & 49 & 5 \\
& DeepSeek-R1 & 0.66 & 1.32 & 1.00 & 0.94 & 0 & 70 & 10 \\
& OpenAI-O1 & 0.51 & 1.07 & 1.00 & 0.71 & 0 & 56 & 4 \\
\midrule
\multirow{4}{*}{\textit{Evolve}} 
& Llama 3.1-405B & 1.20 & 10.4 & 1.08 & 1.01 & 1.00 & 100 & 50 \\
& DeepSeek-V3 & 1.36 & 10.6 & 1.38 & 1.13 & 1.02 & 100 & 68 \\
& DeepSeek-R1 & 1.78 & 27.8 & 1.67 & 1.21 & 1.03 & 100 & 80 \\
& OpenAI-O1 & 1.43 & 11.1 & 1.50 & 1.20 & 1.02 & 100 & 77 \\
\midrule
\multirow{6}{*}{\textit{CUDA-L1}} 
& Stage 1 & 0.94 & 1.39 & 1.00 & 1.00 & 0.98 & 96 & 24 \\
& Stage 1+2 & 1.39 & 10.8 & 1.33 & 1.08 & 1.00 & 100 & 74 \\
& Stage 1+2+GRPO & 3.77 & 39.2 & 2.33 & 1.47 & 1.13 & 100 & 98 \\
& 3 stages - random & 3.22 & 38.6 & 2.25 & 1.32 & 1.10 & 100 & 96 \\
& \quad - island & 6.21 & \textbf{114} & 4.50 & 1.62 & 1.18 & \textbf{100} & 97 \\
& \quad - bucket & \textbf{6.39} & 111 & \textbf{4.42} & \textbf{1.61} & \textbf{1.24} & \textbf{100} & \textbf{97} \\
\midrule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Level 3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{9}{c}{\textbf{Level 3}} \\
\midrule[0.8pt]
\multirow{2}{*}{\textbf{Methods}} & 
\multirow{2}{*}{\textbf{Model}} & 
\multirow{2}{*}{\textbf{Mean}} & 
\multirow{2}{*}{\textbf{Max}} & 
\multirow{2}{*}{\textbf{75\%}} &
\multirow{2}{*}{\textbf{50\%}} &
\multirow{2}{*}{\textbf{25\%}} & 
\textbf{Success}$\uparrow$ & \textbf{Speedup}$\uparrow$ \\
& & & & & & & \small{\# out of 50} & \small{\# out of 50} \\
\midrule
\multirow{4}{*}{\textit{Vanilla}} 
& Llama 3.1-405B & 0.41 & 1.02 & 1.00 & 0 & 0 & 21 & 3 \\
& DeepSeek-V3 & 0.51 & 1.16 & 1.00 & 0.73 & 0 & 26 & 4 \\
& DeepSeek-R1 & 0.80 & 1.47 & 1.00 & 1.00 & 0.97 & 40 & 10 \\
& OpenAI-O1 & 0.71 & 1.47 & 1.00 & 1.00 & 0 & 36 & 8 \\
\midrule
\multirow{4}{*}{\textit{Evolve}} 
& Llama 3.1-405B & 1.17 & 3.00 & 1.19 & 1.03 & 1.00 & 49 & 32 \\
& DeepSeek-V3 & 7.24 & 276 & 1.93 & 1.47 & 1.11 & 49 & 39 \\
& DeepSeek-R1 & 11.8 & 329 & 2.37 & 1.60 & 1.17 & 50 & 43 \\
& OpenAI-O1 & 10.6 & 329 &2.11 & 1.53 & 1.13 & 50 & 43 \\
\midrule
\multirow{6}{*}{\textit{CUDA-L1}} 
& Stage 1 & 0.98 & 1.47 & 1.01 & 1.00 & 1.00 & 47 & 13 \\
& Stage 1+2 & 10.3 & 315 & 1.97 & 1.53 & 1.12 & 49 & 40 \\
& Stage 1+2+GRPO & 31.4 & 426 & 9.96 & 2.23 & 1.27 & 50 & 49 \\
& 3 stages - random & 26.8 & 344 & 9.31 & 2.00 & 1.21 & 50 & 48 \\
& \quad - island & \textbf{52.1} & \textbf{452} & 23.4 & 2.58 & 1.21 & \textbf{50} & 49 \\
& \quad - bucket & 50.8 & 449 & \textbf{22.9} & \textbf{2.66} & \textbf{1.58} & \textbf{50} & \textbf{49} \\
\bottomrule[1.2pt]
\end{tabular}
\end{adjustbox}
\caption{Model performance on KernelBench across level 1, 2 and 3 subsets.}
\label{level-results}

\end{table*}

==> tables/prompt_contrastive_rl.tex <==
\begin{table}[htbp]
  \centering


  %============================= Outer container (single prompt)
  \begin{tcolorbox}[
    rounded corners,
    arc=3pt,
    enhanced,
    width=0.96\textwidth,
    colframe=black,
    colback=white,
    title=\textbf{CUDA Optimization Task Prompt — Used in Contrastive-RL},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
  ]
    %--------------- Part 1: Task description
    \begin{tcolorbox}[
      sharp corners,
      colframe=taskblue,
      colback=taskblue!5,
      colbacktitle=taskblue!15,
      coltitle=taskblue,
      boxrule=0.4pt,
      title={\textbf{Task for CUDA Optimization}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt,
      breakable
    ]
You are a CUDA programming expert specializing in GPU kernel optimization. Given a reference CUDA implementation, your objective is to create an accelerated version that maintains identical functionality. You will receive previous CUDA implementations accompanied by their performance metrics. Conduct a comparative analysis of these implementations and use the insights to develop optimized and correct CUDA code that delivers superior performance.
.%\vspace{2mm} 
    \end{tcolorbox}

    %--------------- Part 2: Previous CUDA implementation with scores
    \begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Previous Cuda Implementations with Scores}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=1pt,
      bottom=1pt,
      breakable,
      listing options={style=codestyle}
    ]
\begin{lstlisting}[language=C++, basicstyle=\small\ttfamily, style=codestyle, frame=none,framerule=0pt]
// code1 (score1)
__global__ void kernel_v1(float* input, float* output, int N) {
    ...
}

// code2 (score2) 
__global__ void kernel_v2(float* input, float* output, int N) {
    ...
}
// code3 (score3) 
__global__ void kernel_v3(float* input, float* output, int N) {
    ...
}
// code4 (score4) 
__global__ void kernel_v3(float* input, float* output, int N) {
    ...
}
\end{lstlisting}
    \end{tcolorbox}

    %--------------- Part 3: Generation protocol
    \begin{tcolorbox}[
      sharp corners,
      colframe=subviolet,
      colback=subviolet!6,
      colbacktitle=subviolet!15,
      coltitle=subviolet,
      boxrule=0.4pt,
      title={\textbf{Generation Protocol}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt,
      breakable
    ]
You MUST use exactly two hash symbols (\#\#) at the beginning of each section. \\
%\vspace{0.1mm}
 \textbf{\#\# Performance Analysis}: Compare code snippets above and articulate on :
\begin{enumerate}[leftmargin=*,noitemsep]
\item Which implementations demonstrate superior performance and why?
\item What particular optimization strategies exhibit the greatest potential for improvement?
\item What are the primary performance limitations in the implementation?
\item What CUDA-specific optimization techniques remain unexploited?
\item Where do the most significant acceleration opportunities exist?
\end{enumerate}
\vspace{0.3mm}
\textbf{\#\# Algorithm Design}: Describe your optimization approach \\
%\vspace{0.3mm}
\textbf{\#\# Code Implementation}: Provide your improved CUDA kernel

\end{tcolorbox}
  \end{tcolorbox}
  \caption{Prompt structure for CUDA optimization task showing reference implementations and their performance scores used in Contrastive-RL.}
\label{tab:cuda-optimization-task}
\end{table}


==> tables/prompt_contrastive_rl_v2.tex <==
\begin{table}[htbp]
  \centering


  %============================= Outer container (single prompt)
  \begin{tcolorbox}[
    rounded corners,
    arc=3pt,
    enhanced,
    width=0.96\textwidth,
    colframe=templateblue,
    colback=white,
    title=\textbf{CUDA Optimization Task Prompt — Used in Contrastive-RL},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
  ]
    %--------------- Part 1: Task description
    \begin{tcolorbox}[
      sharp corners,
      colframe=taskblue,
      colback=taskblue!5,
      colbacktitle=taskblue!15,
      coltitle=taskblue,
      boxrule=0.4pt,
      title={\textbf{Task for CUDA Optimization}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt,
      breakable
    ]
      You are an expert in CUDA programming and GPU kernel optimization. 
      Your task is to analyze and improve existing CUDA implementations based on their performance scores. %\vspace{2mm} 
    \end{tcolorbox}
 %--------------- Part 2-0: Reference Code implementation with scores
    \begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Reference Code}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=1pt,
      bottom=1pt,
      breakable,
      listing options={style=codestyle}
    ]
\begin{lstlisting}[language=C++, basicstyle=\small\ttfamily, style=codestyle, frame=none,framerule=0pt]
__global__ void kernel_v1(float* input, float* output, int N) {
    // Baseline implementation
    ...
}
}
\end{lstlisting}
    \end{tcolorbox}
    
    %--------------- Part 2: Previous CUDA implementation with scores
    \begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Previous Cuda Implementations with Scores}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=1pt,
      bottom=1pt,
      breakable,
      listing options={style=codestyle}
    ]
\begin{lstlisting}[language=C++, basicstyle=\small\ttfamily, style=codestyle, frame=none,framerule=0pt]
// code1 (score1)
__global__ void kernel_v1(float* input, float* output, int N) {
    // Baseline implementation
    ...
}

// code2 (score2) 
__global__ void kernel_v2(float* input, float* output, int N) {
    // Optimized memory access
    ...
}
\end{lstlisting}
    \end{tcolorbox}

    %--------------- Part 3: Generation protocol
    \begin{tcolorbox}[
      sharp corners,
      colframe=subviolet,
      colback=subviolet!6,
      colbacktitle=subviolet!15,
      coltitle=subviolet,
      boxrule=0.4pt,
      title={\textbf{Generation Protocol}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt,
      breakable
    ]
You MUST use exactly two hash symbols (\#\#) at the beginning of each section. \\
%\vspace{0.1mm}
 \textbf{\texttt{\#\# Performance Analysis}}: Compare code snippets above and articulate on :
\begin{enumerate}[noitemsep]
\item  Which implementations demonstrate superior performance and why?
\item What particular optimization strategies exhibit the greatest potential for improvement?
\item What are the primary performance limitations in the implementation?
\item What CUDA-specific optimization techniques remain unexploited?
\item Where do the most significant acceleration opportunities exist?
\end{enumerate}
\vspace{0.3mm}
\textbf{\texttt{\#\# Algorithm Design}}: Describe your optimization approach \\
%\vspace{0.3mm}
\textbf{\texttt{\#\# Code Implementation}}: Provide your improved CUDA kernel

\end{tcolorbox}
  \end{tcolorbox}
  \caption{Prompt structure for CUDA optimization task showing reference implementations and their performance scores used in Contrastive-RL.}
\label{tab:cuda-optimization-task}
\end{table}


==> tables/prompt_sft_aug.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|>{\columncolor{taskblue!20}}p{0.9\textwidth}|}
\hline
\vspace{2mm}
\textbf{\color{taskblue}Task for CUDA Optimization} \\
\vspace{1mm}
You are an expert in CUDA programming and GPU kernel optimization. Now you're tasked with developing a high-performance cuda implementation of Softmax. The implementation must: \\
\begin{itemize}
    \item Produce \textbf{identical} results to the reference PyTorch implementation.
    \item Demonstrate \textbf{speed improvements} on GPU.
    \item Maintain \textbf{stability} for large input values.
\end{itemize}
\vspace{2mm} \\
\hline
\end{tabular}

\vspace{1mm}

\begin{tabular}{|>{\columncolor{refgreen!20}}p{0.9\textwidth}|}
\hline
\vspace{2mm}
\textbf{\color{refgreen}Reference Implementation (exact copy)} \\
\begin{lstlisting}[language=Python, basicstyle=\small\ttfamily]
import torch
import torch.nn as nn

class Model(nn.Module):
    """
    Simple model that performs a Softmax activation.
    """
    def __init__(self):
        super(Model, self).__init__()

    def forward(self, x: torch.Tensor) -> torch.Tensor:
        """
        Applies Softmax activation to the input tensor.
        Args:
            x (torch.Tensor): Input tensor of shape (batch_size, num_features).
        Returns:
            torch.Tensor: Output tensor with Softmax applied, same shape as input.
        """
        return torch.softmax(x, dim=1)

batch_size = 16
dim = 16384

def get_inputs():
    x = torch.randn(batch_size, dim)
    return [x]

def get_init_inputs():
    return []  # No special initialization inputs needed
\end{lstlisting}
\vspace{2mm} \\
\hline
\end{tabular}
\end{center}
\caption{Prompt illustration for data augmentation in Section \ref{sft}. For each KernelBench task (softmax shown here for illustration), the prompt is fed to each of six LLM models—GPT-4o, OpenAI-o1, DeepSeek-R1, DeepSeek V3, Llama 3.1-405B Instruct, and Claude 3.7 Sonnet—to generate alternative CUDA implementations. }
\end{table}

==> tables/prompt_table_template.tex <==
\begin{table}[htbp]
  \centering
  \caption{Prompt illustration for data augmentation in Section~\ref{sft}. The three color‑coded panels below are \emph{components of a single prompt} used for KernelBench tasks (Softmax shown here). The complete prompt is fed to six LLM models—GPT‑4o, OpenAI‑o1, DeepSeek‑R1, DeepSeek V3, Llama 3.1‑405B Instruct, and Claude 3.7 Sonnet—to generate alternative CUDA implementations.}
  \label{tab:prompt-softmax}

  % ============================= Outer container (single prompt)
  \begin{tcolorbox}[
    rounded corners,
    arc=3pt,
    enhanced,
    breakable,
    width=0.96\textwidth,
    colframe=black,
    colback=white,
    title=\textbf{Softmax CUDA Kernel Prompt — Three Complementary Parts},
    fonttitle=\bfseries\large,
    boxrule=0.6pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
  ]
    % --------------- Part 1: Task description
    \begin{tcolorbox}[
      sharp corners,
      colframe=taskblue,
      colback=taskblue!5,
      colbacktitle=taskblue!15,
      coltitle=taskblue,
      boxrule=0.4pt,
      title={\textbf{Task for CUDA Optimization}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt
    ]
      You are an expert in CUDA programming and GPU kernel optimization. Your goals are:
      \begin{itemize}[leftmargin=*]
        \item Produce \textbf{identical} results to the reference PyTorch implementation.
        \item Demonstrate \textbf{speed improvements} on GPU.
        \item Maintain \textbf{stability} for large input values.
      \end{itemize}
    \end{tcolorbox}

    %\bigskip

    % --------------- Part 2: Previous CUDA implement with scores
    \begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Previous CUDA Implementation with Scores}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt
    ]
      \begin{center}
        \begin{lstlisting}[style=codestyle, frame=none,framerule=0pt]
#include <float.h>
#include <cuda_runtime.h>

__global__ void softmax_kernel(const float* __restrict__ in,
                               float* __restrict__ out,
                               int dim) {
    extern __shared__ float smem[];
    int row = blockIdx.x;            // each block handles one row
    int tid = threadIdx.x;
    float max_val = -FLT_MAX;
    __syncthreads();
    for (int offset = blockDim.x / 2; offset > 0; offset >>= 1) {
        if (tid < offset) smem[tid] += smem[tid + offset];
        __syncthreads();
    }
    sum = smem[0];

    // 3) write normalized values
    for (int i = tid; i < dim; i += blockDim.x) {
        out[row * dim + i] = smem[i] / sum;
    }
}
\end{lstlisting}
      \end{center}
      %\medskip
      %\textit{Note:} The scores are measured on an NVIDIA A100 (80GB, CUDA 12.4) with batch size =~1024 and feature dimension =~65,536.
    \end{tcolorbox}

    % \bigskip

    % --------------- Part 3: Generation protocol
    \begin{tcolorbox}[
      sharp corners,
      colframe=subviolet,
      colback=subviolet!6,
      colbacktitle=subviolet!15,
      coltitle=subviolet,
      boxrule=0.4pt,
      title={\textbf{Generation Protocol}},
      fonttitle=\bfseries,
      left=4pt,
      right=4pt,
      top=4pt,
      bottom=4pt
    ]
      \begin{itemize}[leftmargin=*]
        \item \textbf{Input}: The entire prompt (Parts 1–3) is passed verbatim to the target LLM.
        \item \textbf{Output format}: The model must return a complete, self‑contained CUDA source file (`.cu`) followed by a short Markdown block with build and run commands.
        \item \textbf{Time limit}: Generation should complete within 120 seconds.
        \item \textbf{Forbidden}: Any network access, dynamic code execution, or external dependencies beyond CUDA and C++ standard libraries.
      \end{itemize}
    \end{tcolorbox}
  \end{tcolorbox}
\end{table}


